The cool and the cruel: separating hard parts of LWE secrets

Sparse binary LWE secrets are under consideration for standardization for Homomorphic Encryption and its applications to private computation. Known attacks on sparse binary LWE secrets include the sparse dual attack and the hybrid sparse dual-meet in the middle attack which requires significant memory. In this paper, we provide a new statistical attack with low memory requirement. The attack relies on some initial lattice reduction. The key observation is that, after lattice reduction is applied to the rows of a q-ary-like embedded random matrix $\mathbf A$, the entries with high variance are concentrated in the early columns of the extracted matrix. This allows us to separate out the "hard part" of the LWE secret. We can first solve the sub-problem of finding the "cruel" bits of the secret in the early columns, and then find the remaining "cool" bits in linear time. We use statistical techniques to distinguish distributions to identify both the cruel and the cool bits of the secret. We provide concrete attack timings for recovering secrets in dimensions $n=256$, $512$, and $768$. For the lattice reduction stage, we leverage recent improvements in lattice reduction (e.g. flatter) applied in parallel. We also apply our new attack in the RLWE setting for $2$-power cyclotomic rings, showing that these RLWE instances are much more vulnerable to this attack than LWE.

==> AFRICACRYPT_SUBMISSION/Makefile <==
LATEX=latex
BIBTEX=bibtex
BIBFILE=references.bib
PAPER=picante

TEXFILES = picante.tex \
	intro.tex \
	back.tex \
	method.tex \
	attack.tex \
	results.tex \
	discussion.tex \

EPSFIGS = \

EPSGRAPHS = $(wildcard figures/*.eps)

all:   $(PAPER).pdf

subdirs:
	$(MAKE) -C figure

bib:
	$(BIBTEX) (PAPER)

%.eps: %.fig
	fig2dev -L eps $< $@

$(PAPER).ps: $(PAPER).dvi
	dvips -Ppdf -Pcmz -Pamz -t letter -D 600 -G0 -f $(PAPER).dvi > $(PAPER).ps

#$(PAPER).pdf: $(PAPER).dvi
#	dvipdf $(PAPER).dvi

# if need to embed font
$(PAPER).pdf: $(PAPER).ps
	ps2pdf14 -dEmbedAllFonts=true -dPDFSETTINGS=/prepress $(PAPER).ps

$(PAPER).dvi: $(EPSFIGS) $(TEXFILES) $(BIBFILE)
	$(LATEX)  $(PAPER)
	$(BIBTEX) $(PAPER)
	$(LATEX) $(PAPER)
	$(LATEX)  $(PAPER)

$(PAPER).blg: $(BIBFILE)
	$(LATEX)  $(PAPER)
	$(BIBTEX) $(PAPER)
	$(LATEX)  $(PAPER)

clean:
	/bin/rm -f *.dvi *.aux *.ps *~ *.log *.lot *.lof *.toc *.blg *.bbl *.pdf *.out


==> AFRICACRYPT_SUBMISSION/attack.tex <==
\section{Related Work}
\label{sec:compare}
Albrecht et al \cite{albrecht2018} classify attacks on LWE broadly into primal \cite{LP11,LN13,AFG13} and dual \cite{MR09,Albrecht2017_sparse_binary} attacks.
Some primal attacks reduce search-LWE (see \cref{sec:attack} for definition) to the unique shortest vector problem (uSVP) and solve this via lattice reduction \cite{albrecht2017revisiting}. Others employ a combination of lattice reduction and Bounded Distance Decoding (BDD) \cite{LP11}. The goal of dual attacks is to solve Decision-LWE (see \cref{sec:attack}) by reducing it to the Shortest Integer Solution (SIS) problem \cite{ajtai1996generating}, further reduced into the problem of finding short vectors in the dual lattice defined by $\{ x \in \mathbb{Z}^m_q | Ax = 0 \mod q \}$.

\para{Hybrid attacks.} The notion of hybrid attacks was introduced in 2007 by \cite{howgrave2007hybrid}, who proposed combining lattice reduction and meet-in-the-middle (MITM) attacks against NTRUEncrypt. \cite{buchmann2016} extended this idea to binary-error LWE.
A collection of such hybrid attacks have been proposed for different LWE settings.
\cite{bilu2021} provide a succinct overview in their Table 1.
\cite{soncheon2019} succeeded in applying a hybrid attack to settings of sparse ternary secrets with small error via a primal attack strategy.
\cite{Albrecht2017_sparse_binary} was the first work to combine the notions of hybrid attacks in the dual lattice for sparse binary and ternary secrets and small error.
The attack benefits from optimizing a trade-off between success probability by guessing parts of the secret and performing the costly lattice reduction on the now lower-dimensional lattice. 
\cite{Cheon_hybrid_dual} improved upon \cite{Albrecht2017_sparse_binary} by using MITM for the guessing part.
\cite{espitau2020} optimized further by recognizing an inefficiency in the matrix multiplication during the guessing and considered small, non-sparse secrets.
\cite{bilu2021} extended this line of attack to arbitrary secrets and find that ``hybrid dual attacks [usually] outperform [non-hybrid] dual attacks regardless of the secret distribution''.

\para{Our work.} In contrast to (but not necessarily incompatible with) work in hybrid attacks, our attack performs the lattice reduction on a full-sized lattice using different subsets of available LWE samples. Our lattice is endowed with a scaling (or penalty) parameter $\omega$. The scaling is similar to the scaling used in \cite{bai_galbraith,Albrecht2017_sparse_binary}, and its utility is discussed in \cref{sec:reduction}.
Our key insight, the non-uniformity over coordinates in the reduced basis, naturally splits the problem into two parts (in this case the ``cruel'' and ``cool'' bits), reminiscent of a hybrid attack.

%\para{Hybrid attacks.} Our attack follows a similar pattern to so-called ``hybrid attacks'', which leverage an initial step of lattice reduction followed by a meet-in-the-middle attack~\cite{JFRT16}, \cite{HG07}. There are two key differences. 
%First, our observation about the shape of the reduced $\mathbf{RA}$ matrix allows us to precisely fix the ``meet-in-the-middle'' dimension, since we know which columns are hard, and which are easy. Second, combining our observation about the shape leads to a novel attack which demonstrates that (2-cyclotomic) RLWE is strictly weaker than LWE.
%
%Our attack is different from Albrecht’s~\cite{Albrecht2017_sparse_binary} dual attack on sparse secrets, which chooses some subset of the columns to reduce.  If all columns not included in that set happen to correspond to zero bits in the secret (which will happen with some known probability for sparse binary secrets), then the LWE instance can be distinguished from random using the dual attack on the smaller dimensional LWE instance corresponding to the selected columns.  But if any of the other bits were active bits, then the distinguisher will fail.
%%
%Interestingly, one can think of our attack as “reduce, then separate according to reduction” as opposed to the attack in~\cite{Albrecht2017_sparse_binary}, which does “separate via random guess, then reduce”. 
%A variant of~\cite{Albrecht2017_sparse_binary}, referred to as the dimension-error trade-off, discussed extensively in~\cite{Cheon_hybrid_dual}, includes the possibility to exhaustively search through non-zero secret guesses for the chosen remaining columns, at the expense of a large memory requirement.  This version does not have the benefit that our attack enjoys, which is that we separate out the cool bits from the cruel bits via our reduction step to start with. 
%
%In our approach, we first reduce the whole matrix $\mathbf A$, then concentrate on the first $n_u$ columns which now correspond to the “cruel” unreduced entries of high variance. Then we solve the reduced LWE problem for those $n_u$ columns and extend to the full secret in linear fashion, as described in Section~\ref{sec:attack}.
%
%The key difference between our attack and ~\cite{Albrecht2017_sparse_binary} is that we separate out the columns of $\mathbf A$ which have high variance after reduction, and this does not depend on where the active bits of $\mathbf s$ are positioned.  
%The ``cool'' columns of $\mathbf A$ won’t contribute much to the noisy inner product even if there are active bits for the secret $\mathbf s$ in those positions.  
%\nolte{quote the 2021 paper}

%Our attack is also different from the hybrid attack on sparse binary secrets presented in~\cite{Cheon_hybrid_dual}, which describes a Meet in the Middle attack for LWE, implemented using a noisy collision search.  The idea is to write a sparse binary secret vector $\mathbf s$ with Hamming weight $h$ as a sum of $\mathbf s_1 + \mathbf s_2$, two vectors each with Hamming weight $\approx h/$2.   Computing a set $\mathcal T$ of $\mathbf A \cdot \mathbf s_1$ for all possible $\mathbf s_1$ (and storing a hash table for look-up), the noisy collision search is used to find an $\mathbf s_2$ such that $b-\mathbf A \cdot \mathbf s_2$ is close to an element of $\mathcal T$.  This noisy collision search is then used as a subroutine of the Hybrid attack which combines two algorithms.
%One algorithm returns a smaller dimensional LWE sample with a larger error, and the other algorithm is a Meet-in-the-middle attack for binary sparse LWE problems.  Combining them yields a hybrid dual attack, which can tolerate wrong guesses for the zero columns at the expense of doing a meet-in-the-middle noisy collision search.  The noisy collision search relies on a very large memory requirement, for example, roughly $2^{75}$ memory requirement for all estimated predicted attack times given in~\cite{Cheon_hybrid_dual}. 

\input{tables/notation} 

\section{The Attack} \label{sec:attack}
The Learning With Errors (LWE) problem, first introduced by Regev~\cite{Reg05}, can be stated in 2 forms. The {\em Search-LWE} problem is: given a random matrix \( \mathbf A \in \mathbb{Z}_q^{m \times n} \), a secret vector \( \mathbf{s} \in \mathbb{Z}_q^n \), and an error vector \( \mathbf{e} \in \mathbb{Z}_q^m \) (usually sampled from some small error distribution), find \( \mathbf{s} \), given $\mathbf A$ and 
\begin{align}
\mathbf{b} = \mathbf A\cdot \mathbf{s} + \mathbf{e} \mod q,
\end{align}
where $m$ denotes the number of LWE samples, $n$ is the lattice dimension, and $q$ is the modulus. In the related {\em Decision-LWE} problem, the objective is not to find the secret vector \( \mathbf{s} \), but to distinguish between two distributions: given a random matrix \( \mathbf A \in \mathbb{Z}_q^{m \times n} \) and a vector \( \mathbf{b} \in \mathbb{Z}_q^m \), decide whether \( \mathbf{b} \) is drawn from the distribution \( \mathbf A\cdot \mathbf{s} + \mathbf{e} \mod q \) for some secret vector \( \mathbf{s} \in \mathbb{Z}_q^n \) and error vector \( \mathbf{e} \in \mathbb{Z}_q^m \), or whether \( \mathbf{b} \) is drawn from the uniform random distribution over \( \mathbb{Z}_q^m. \) \cite{Reg05} showed that for $q$ of size polynomial in $n$, there is a reduction from Search-LWE to Decision-LWE.  See \cref{tab:notation} for notation used in the paper.

 We introduce a new attack on the LWE problem for sparse binary secrets, i.e. $\mathbf{s} \in \{0,1\}^n$, with $h$, the Hamming weight (number of $1$s in $\mathbf s$), small. The attack leverages an observation about the shape of reduced LWE matrices to separate the hard and easy parts of the secret. It works as follows. 

\para{Attack Part 1: Lattice Reduction.} We begin by applying  lattice reduction to (the rows of) an embedding $\mathbf \Lambda \in \mathbb{Z}_q^{(m+n) \times (m+n)}$ of the data:
\begin{align}
\label{eq:embedding}
\mathbf \Lambda = 
\begin{pmatrix}
0 & q \mathbf{I}_n \\
\omega \mathbf{I}_m &\mathbf  A
\end{pmatrix}
\end{align}
The reduction finds a linear transformation $\left[\mathbf{C}, \mathbf{R}\right]$ such that 
%\begin{align}
$\mathbf \Lambda^r = \left[\mathbf{C}, \mathbf{R}\right] \mathbf{\Lambda} =
\left[ \omega \mathbf{R}\mathbf{I}_m, q\mathbf{C}\mathbf{I}_n + \mathbf{RA} \right]$.
%\end{align}
We extract the transformation matrix $\mathbf R = \mathbf \Lambda^r_{*,0:m}/\omega$,
which corresponds to the row and column operations performed to transform the matrix $A$ into its reduced form.
$\mathbf{R}$ is applied to both $\mathbf{A}$ and $\mathbf{b}$ to create reduced sample pairs.
For ease of notation, we will refer to $\mathbf R\mathbf A$ as $\mathbf A$ or ``reduced $\mathbf A$'' and $\mathbf  R \mathbf{b}$ as $\mathbf{b}$ throughout the text, and otherwise specify ``original'' pairs.

Reduction algorithms trade off the error on the reduced LWE pairs for the norm of the rows in reduced $\mathbf A$. The ``penalty parameter'' $\omega$ controls this trade-off, where higher $\omega$ causes less norm and variance reduction, but also less error amplification. Details of lattice reduction can be found in Section \ref{sec:reduction}.



\begin{figure*}[ht!]
   \vspace{-0.4cm}
    \centering
    \subfigure[]{\includegraphics[width=0.45\textwidth]{figs/n256_q12.pdf}} 
 %   \subfigure[]{\includegraphics[width=0.4\textwidth]{figs/n256_q20.pdf}} 
    \subfigure[]{\includegraphics[width=0.45\textwidth]{figs/n512_logq28_red.pdf}}
    \subfigure[]{\includegraphics[width=0.45\textwidth]{figs/n512_q41.pdf}}
    \subfigure[]{\includegraphics[width=0.45\textwidth]{figs/n768_q35.pdf}}
    \vspace{-0.2cm}
    \caption{The standard deviation of elements within each column of the $\mathbf{A}$ matrix before and after reduction (and extraction from the q-ary embedding) for various $n$/$q$ settings. The first $n_u$ unreduced columnms (left half of the figures) correspond to the ``cruel'' bits of the secret, while the remaining $n_r = n - n_u$ are the ``cool'' bits.  This phenomenon is distinct from the "z-shape" exhibited by the Gram-Schmidt orthogonalized rows of a q-ary lattice before and after lattice reduction~\cite{howgrave2007hybrid,albrecht2021lattice} (see Appendix~\ref{subsec:zshape} for details).
    }
    \label{fig:stdev_examples}
    \vspace{-0.5cm}
\end{figure*}



\para{Attack Part 2: Identify Cruel and Cool Bits.} The key observation of this attack is that the resulting reduced $\mathbf{A}$ samples all share a reduction pattern: 
\begin{formal} 
{\bf Key observation:} {\it The first $n_u$ elements of each sample vector  $\mathbf A_{*,0:n_u}$ remain unreduced and retain their uniform distribution over $\mathbb{Z}_q$,
and all subsequent $n_r = n - n_u$ elements of $\mathbf A_{*, n_u:n}$ are heavily reduced. }
\end{formal}

To illustrate this key observation, we plot the standard deviation over columns in $\mathbf A$ against the column index in \cref{fig:stdev_examples} for various $n$ and $\log_2 q$ settings. %This pattern seems to be a direct consequence of the embedding in \cref{eq:embedding}. %We believe that our choice for the penalty parameter is one cause for this observation.
%
%\kl{the next few sentences are confusing adn seem to mix several different messages together.  What is the point here? I would comment them out until the last sentence, and move them somewhere else.} By permuting columns of $\mathbf A$ or $q\mathbf I_n$, we can achieve the reduction on any column subset of size $n_r$ in $\mathbf A$. Moreover, due to the algebraic structure of 2-power cyclotomic RLWE, one can shift the columns of $\mathbf A$ by any offset. This reveals a vulnerability of the sparse secrets because we can perform a brute force attack up to a much lower hamming weight. $\omega$ then controls the trade-off between $n_u$ and the size of the error. 
This observation of cruel and cool bits inspires the following hypothesis:
 
\begin{formal}
{\bf Hypothesis:} For any row $\mathbf a$ of $\mathbf A$, the $n_r$ last entries contribute comparatively little to the overall dot product $\mathbf a \cdot \mathbf s$. Thus, for a sparse enough secret, the Decision-LWE may be solvable without correctly guessing the $n_r$ secret bits.\end{formal}
In other words, this shape resulting from lattice reduction means we only need to solve LWE on a smaller dimension $n_u < n$. In essence, \textit{we separate out the hard part of the LWE secret at the cost of increased error}. We validate this hypothesis in the remainder of this paper. In the framing of the distinguishing attack \cite{MR09,RS10}, we leverage lattice reduction to boost the distinguishing advantage specifically on the cool bits.

\para{Attack Part 3: Secret Guessing.} Next, we leverage statistical properties of the cool and cruel regions to guess the secret. Figure \ref{fig:as-bmodq} shows a histogram of the distribution of the residuals $\mathbf a\cdot \mathbf{s} - b \mod q$ (in blue) and $\mathbf a\cdot \mathbf{s}^* - b \mod q$ (in orange), where $\mathbf{s}^*$ shares the first $n_u$ with $\mathbf{s}$
and has all other $n_r$ elements set to $0$. Green corresponds to a random guess for the secret with equal hamming weight. The orange and the green distributions are distinct, enabling us to detect the correctness of the first $n_u$ bits in the secret without knowing the others. Given the size of the error on the reduced LWE problem, so far we have not found a more efficient attack for guessing the first $n_u$ secret bits than brute force. One could think of using one of the hybrid attack strategies outlined in the related work on the cruel part, but we leave this for future work.
%the large error may  prohibit this.

\begin{figure}[h]
    \centering
    \includegraphics[width=0.65\linewidth]{figs/distributions.pdf}
    \caption{Histogram of 4 million samples of the residual $(\mathbf a \cdot \mathbf{s^*} - b) \mod q$ (centered and normalized) for different secret guesses $\mathbf{s^*}$ ($n=512$, $\log_2 q = 41$, $h=20$). The three histograms correspond to three different guesses. Blue corresponds to the true secret, orange to the secret candidate that has only the first $n_u=75$ bits correct and green to a random secret with $h=20$. The numbers in the legend correspond to the sample standard deviation relative to the uniform standard deviation $\frac{q}{\sqrt{12}}$.
    }
    \label{fig:as-bmodq}
    \vspace{-0.3cm}
\end{figure}

Given a secret guess $\mathbf{s}^*$ with correct $n_u$ cruel bits, the $n_r$ remaining cool bits can be recovered easily, given enough samples. One fast method is greedy recovery, presented in Algorithm \ref{alg:greedy_cool}. It works as follows: 
start with a candidate secret 
$\mathbf{s}^*$ which shares the first $n_u$ cruel bits with $\mathbf{s}$
and has all other $n_r$ bits set to $0$.
Starting with the first cool bit, flip that bit of $\mathbf{s}^*$ to $1$. Then calculate if this flip increases the 
standard deviation of the resulting 
$\mathbf a \cdot \mathbf{s}^* - {b} \mod q$ (over $m$ reduced samples $(\mathbf a,b)$). If so, flip it back to $0$ and move to the next bit. Note the standard deviation here is a practical proxy for a proper statistical test. Section \ref{sec:practical} expands on this. Intuitively, greedy recovery works because every correct bit flipped to 1 will reduce the orange distribution in Figure \ref{fig:as-bmodq} closer to the blue and every wrong one will introduce more noise, sending it closer to the green. 
%\begin{wrapfigure}{r}{0.3\textwidth}
 %\begin{minipage}{0.5\textwidth}
\begin{algorithm}
\caption{Greedy recovery of cool bits}\label{alg:greedy_cool}
\begin{algorithmic}[1]
\For{ $i \in n - n_r : n$}
    \State $ \mathbf{s}^*[i] \gets 0 $
    \State $ \sigma_0 \gets \sigma(\mathbf a \cdot \mathbf{s}^* - {b} \mod q)$ 
    \State $ \mathbf{s}^*[i] \gets 1 $
    \State $ \sigma_1 \gets \sigma(\mathbf a \cdot \mathbf{s}^* - {b} \mod q)$ 
    \If{$ \sigma_0 \leq \sigma_1 $}
        \State $ \mathbf{s}^*[i] \gets 0 $
    %    \State \text{continue}
    \Else
        \State $ \mathbf{s}^*[i] \gets 1 $
    \EndIf
\EndFor
\end{algorithmic}
\end{algorithm}
\vspace{-0.5cm}
%\end{minipage}
%\end{wrapfigure}

Otherwise, one can employ more principled gradient-free optimization methods, like simulated annealing. Annealing works better with limited data, but is slower. The best choice depends on the setting.
All methods work efficiently due to the reduced variance of the corresponding entries in $\mathbf A$. 
%Intuitively, one can think of the LWE as much closer to a linear regression problem when the entries entries of $\mathbf A$ are sufficiently reduced. In conclusion, we can view the original LWE problem as reduced to a second, lower dimensional LWE problem with much larger error.



%KL: can this go into the Greedy algorithm somehow? 
% The std function evaluated the standard deviation over the LWE samples.


\subsection{Practical considerations} \label{sec:practical}
\vspace{-0.1cm}

\para{Implementation.} As described in detail in Section \ref{sec:reduction}, we sample views of the $4\cdot n$ sized lattice defined by the LWE samples and reduce them individually, forming a large set of reduced LWE samples for use in the attack, following~\cite{picante,verde}. After identifying the cool and cruel bits, secret recovery runs in two parts: first, guessing the cruel secret bits on the the reduced LWE problem with large error, then the recovery of the full secret via Algorithm \ref{alg:greedy_cool}.

We use brute force enumeration for cruel secret bit recovery. All code is implemented in Python, and we employ GPU acceleration via \texttt{pytorch} \cite{pytorch}.
Batches of secret candidates are continuously sent to the device and evaluated on a suitable amount of data to distinguish the residuals $\mathbf A\cdot \mathbf{s}^* - \mathbf{b} \mod q$ if the true (part of the) secret was found, see the orange histogram in Figure \ref{fig:as-bmodq}.
Since our brute force is perfectly parallelizable, we can distribute the work to an arbitrary number of GPUs or CPUs. Candidate secrets are enumerated in ascending Hamming weight, and a record of the top-$k$ candidates, according to a metric defined below, are evaluated at constant intervals throughout the enumeration. Evaluation involves running Algorithm \ref{alg:greedy_cool} and then checking if the resulting secret produces nearly correct ($\mathbf{A, b}$) pairs.
The evaluation frequency can be traded off against the amount of data used during enumeration and $k$, the number of candidates kept in the top-$k$ set.

\para{Candidate Evaluation.} The metric by which candidate secrets are sorted can involve any test that distinguishes from uniformity in the residual, but in practice it must be fast. Most non-parametric tests like Kolmogorov-Smirnov or Kuiper involve calculating a Cumulative Distribution Function (CDF) and thus sort the data, which is slow.
A likelihood ratio test is generally more powerful, but evaluating such a test on a distribution modulo $q$ involves evaluation over multiple ``wraps'' around the modulus.
Under certain assumptions, detailed in Section \ref{sec:theory}, the distribution we aim to distinguish from uniform is a mod-Gaussian involving an infinite sum:
\begin{align}
f(x) \propto \sum_{k=-\infty}^{\infty} \mathcal{N}(x ; \mu + k\cdot q, \sigma^2).
\end{align}
Even with suitable truncation, the runtime of a likelihood ratio test will at best be $O(N\cdot K)$ with $N$ samples and truncation to $K$ elements of the sum.
\cite{espitau2020} also explores a way of specifically distinguishing modular Gaussians via a periodic aggregation metric $Y=\sum^N_{i=1} \exp(2\pi iX_i)$, see their Algorithm 2.
We thought, since both distributions, uniform and mod-Gaussian are fully defined by their first two moments and have their mean fixed to the same value, a direct comparison of the second moment suggests itself as a simple but powerful distinguishing method.
Thus, we choose the direct variance comparison described in Algorithm~\ref{alg:greedy_cool} due to its simplicity and computational efficiency. Empirically, we found that it was similarly powerful to a Kuiper test, and more than 5x faster in the settings considered.

\para{Other performance considerations.}
Values of $\mathbf A, \mathbf b$ are of the order of $q$ and thus large in the considered scenarios. However, high precision is not needed during the enumeration and evaluation, since all precision is drowned out by the large error. Since modern GPUs work best with 16-bit floating point numbers, we scale all values down to a range appropriate for those representations. We also employ \texttt{pytorch}  compilation to alleviate some of the overhead of python being an interpreted language. This feature compiles, optimizes and fuses tensor operations, giving a 2-3x speed improvement over the default eager execution.

Our implementation can evaluate roughly 5 billion secrets of dimension $n=512$ through an NVIDIA V100 GPU in about 1 hour during the brute force search. The greedy secret recovery step is fast and runs infrequently. Additional speedups can be had with additional optimizations, such as the use of dedicated CUDA kernels. % We haven't made specific optimizations to the code, for instance dedicated CUDA kernels, so speed-ups are to be expected from a better implementation.
Additionally, our attack does not yet exploit the recursive search space structure trick from \cite{espitau2020}.


==> AFRICACRYPT_SUBMISSION/discussion.tex <==
%Our attack is also different from the hybrid attack on sparse binary secrets presented in~\cite{Cheon_hybrid_dual}, which describes a Meet in the Middle attack for LWE, implemented using a noisy collision search.  The idea is to write a sparse binary secret vector $\mathbf s$ with Hamming weight $h$ as a sum of $\mathbf s_1 + \mathbf s_2$, two vectors each with Hamming weight $\approx h/$2.   Computing a set $\mathcal T$ of $\mathbf A \cdot \mathbf s_1$ for all possible $\mathbf s_1$ (and storing a hash table for look-up), the noisy collision search is used to find an $\mathbf s_2$ such that $b-\mathbf A \cdot \mathbf s_2$ is close to an element of $\mathcal T$.  This noisy collision search is then used as a subroutine of the Hybrid attack which combines two algorithms.
%One algorithm returns a smaller dimensional LWE sample with a larger error, and the other algorithm is a Meet-in-the-middle attack for binary sparse LWE problems.  Combining them yields a hybrid dual attack, which can tolerate wrong guesses for the zero columns at the expense of doing a meet-in-the-middle noisy collision search.  The noisy collision search relies on a very large memory requirement, for example, roughly $2^{75}$ memory requirement for all estimated predicted attack times given in~\cite{Cheon_hybrid_dual}. 


\section{Discussion and Future Work}

%\begin{itemize}
%\item Trade-off reduction/error when recovering cool bits
%\item Role of GPU
%\item improving  cool bit recovery
%\item Comparison with other attacks
%\end{itemize}
We have presented an attack on Learning With Errors in the setting of sparse binary secrets. Our key insight is the reduction of the LWE problem to one of smaller dimension via lattice reduction and sufficient subsampling.
We discuss the attack empirically and theoretically and highlight actual successful attacks on problem scales up to $n=768$. We leave several important tasks as future work.

\para{Improving upon combinatorial scaling in reduced problem.} We use brute force to solve the smaller LWE problem (e.g. in the cruel region).
This is the crudest way to solve this problem, albeit perfectly parallelizable. The guessing parts of hybrid attack strategies of related work could speed up enumeration. One related way in which we already exploit this is in the 2-cyclotomic RLWE setting.
But of course, the rotation (or more generally, permutation) of the cruel bit region can of course be done on the LWE settings as well. We did not elaborate on that (hybrid) approach because it requires re-reduction of lattices.

\para{Balancing reduction and secret recovery costs.} Currently, our attack runs lattice reduction until it stalls for a given $n$/$q$ setting, then runs secret recovery for the highest $h$ that can be achieved in reasonable time. In the future, our attack should balance the reduction and enumeration costs given the setting of concern, also depending on how hybrid attacks will be employed.

\para{Recovering the cool bits.} As Section~\ref{sec:cool_bits} demonstrates, cool bit recovery is somewhat sample-inefficient, because \cref{alg:greedy_cool} must distinguish between $F_q(k\sigma_r^2+\sigma_e^2)$ and $F_q((k+1)\sigma_r^2+\sigma_e^2)$. This difference tends to be small when $k$ is large, and $\sigma_e$ is large, compared to $\sigma_r$, necessitating more samples. This suggests an additional consideration for the lattice reduction phase: balancing the amount of reduction achieved and the noise added in the process. When reduction factor $\rho$ is smaller, $\sigma_r$ is smaller, resulting in fewer cruel bits and easier recovery. On the other hand, a smaller $\rho$ means a larger $\sigma_e$, necessitating more data during the attack. We leave the quantitative analysis of this relationship as future work.


==> AFRICACRYPT_SUBMISSION/distribution.tex <==
\section{Statistical tests and analysis}
\label{sec:theory}

%\subsection{Statistical calculation of sample size}

Three statistical tests must be performed during the attack: testing whether a brute force guess of the cruel bits is correct, testing whether cool bits are zero or one (in Algorithm~\ref{alg:greedy_cool}), and testing a full secret guess.
% \begin{enumerate}[nosep]
% \item Testing whether a brute force guess of the cruel bits is correct
% \item Testing whether cool bits are zero or one (in Algorithm~\ref{alg:greedy_cool})
% \item Testing a full secret guess.
% \end{enumerate}
The first two tests are performed on reduced LWE samples, obtained during the pre-processing phase. The third involves a simple check of residuals on the original LWE sample and will not be discussed here. We elaborate on the statistical properties of these tests, estimate the number of samples needed, and illustrate our results with concrete attack statistics.

\subsection{Testing brute-forced guesses of the cruel bits} 

Suppose a guess of the cruel bits was made, and let $\mathbf s^*$ be the secret guess derived by setting all cruel bits to their guessed values and all cool bits to zero. We are given $m$ reduced LWE samples $(\mathbf a,b)$, with the same secret $\mathbf s$, error $e$ and reduction factor $\rho$. We consider the random variable $x = \mathbf a \cdot \mathbf s^* - b= \mathbf a \cdot (\mathbf s^* - \mathbf s)-e \mod q,$ centered to $(-\frac q2,\frac q2)$. Our intuition from Section \ref{sec:attack} is that the standard deviation of $x$ (calculated on $m$ reduced samples) will be lowest when all cruel bits are correctly predicted. 

%. Our intuition is that the standard deviation of $x$ will be lower when all cruel bits are correctly predicted. By estimating it on a large enough sample of reduced pairs (i.e. with $m$ large enough), we can build a reliable test. Our goal, here, is to provide a theoretical estimate of $m$.

More precisely, let $n$ be the problem dimension and $n_u$ the number of cruel bits. Over reduced LWE samples $(\mathbf a,b)$, the $n_u$ first coordinates of $\mathbf a$, which correspond to the cruel bits, have standard deviation $\sigma_u=\frac {q}{\sqrt{12}}$ (the standard deviation of the uniform distribution). 
The standard deviation $\sigma_r$ of the $n_r$ remaining coordinates of $\mathbf a$ (the cool bits) can be derived from the reduction factor $\rho$ and $n_u$ under the assumption that all coordinates of $\mathbf a$ are independent after reduction, as follows:
\begin{align}
\rho^2 \sigma_u^2 = \frac{n_u}{n} \sigma_u^2+\frac{n_r}{n}\sigma_r^2,
\end{align}
and therefore %$$\sigma_c^2 = \frac{\rho^2 n - n_a}{n-n_a} \sigma_u^2,$$
\begin{align}
\sigma_r = \sqrt{\frac{\rho^2 n - n_u}{n_r}} \sigma_u.
\end{align}

\noindent Applying these formulas to the examples in Table~\ref{tab:datasets}, we have:
\begin{packed_itemize}
\item $\sigma_r=0.27 \sigma_u$ for $n=256$ and $\log_2 q=12$ ($\rho=0.769$ and $n_u=143$)
\item $\sigma_r=0.15 \sigma_u$ for $n=512$ and $\log_2 q=28$ ($\rho=0.677$ and $n_u=228$)
\item $\sigma_r=0.17 \sigma_u$ for $n=512$ and $\log_2 q=41$ ($\rho=0.413$ and $n_u=75$)
\item $\sigma_r=0.19 \sigma_u$ for $n=768$ and $\log_2 q=35$ ($\rho=0.710$ and $n_u=373$).
\end{packed_itemize}

When all cruel bits are correctly predicted, and if $h_r$ is the number of ones in the $n_r$ cool bits of the secret (a known value since the Hamming weight of the secret is known), the variance of $x$ is
%\begin{align}
$\sigma^2_{\mathcal{G}_q}(x)=F_q(h_r\sigma_r^2 + \sigma_e^2)$,
%\end{align}
with $F_q(v)$ the variance modulo $q$ of a centered Gaussian with variance $v$ and a modular operation. We assume independence in the reduced samples and therefore a Gaussian distribution of $x$ before the modulo operation, %because reduced samples are independent, and therefore 
so the Central Limit Theorem (CLT) holds.

When some cruel bits are incorrect, the residual distribution becomes almost indistinguishable from uniform, because even one incorrect cruel bit significantly increases the Gaussian variance.
%Values of $\frac{\sigma_{\mathcal{G}_q}(x)}{\sigma_u}$ for different $h_r, n$ and $\log_2 q$, calculated by sampling Gaussian variables with the right standard deviation and applying the modulo $q$ operation, are presented in Table~\ref{tab:cruelrecovery}. \todo{FIX TABLE}
%
%\begin{table}[h]
%    \small
%    \vspace{-0.5cm}
%    \centering
%    \caption{\small \textbf{Cruel bit recovery.} Ratio of standard deviation of $\mathbf a \cdot \mathbf s^* -b$, when the cruel bits of $\mathbf s^*$ are correct and incorrect ($\sigma_{\mathcal{G}_q}(x)/\sigma_u$), for different values of $h_r$.}
%    \label{tab:cruelrecovery}
%    \vspace{0.1cm}
%    \begin{tabular}{ccc@{\hskip 12pt}ccccc}
%        \toprule
%        & & & \multicolumn{5}{c}{$\sigma_{\mathcal{G}_q}(x)/\sigma_u$}\\
%        \cmidrule(lr){4-8}
%        n& $\log_2 q$ & $\sigma_u$ & $h_r=3$ & $h_r=5$ & $h_r=10$ & $h_r=15$ & $h_r=20$ \\
%        \midrule
%        256 & 12 & $961$ & 0.90 & 0.92 & 0.96 & 0.98 & 0.99\\
%        512 & 28 & $5.2\cdot 10^7$ & 0.72 & 0.74 & 0.79 & 0.83 & 0.86\\
%        768 & 35 & $9.8\cdot 10^9$ & 0.87 & 0.89 & 0.92 & 0.94 & 0.96\\
%       \bottomrule
%    \end{tabular}
%   \vspace{-0.5cm}
%\end{table}

\para{Samples needed for cruel bit recovery.} We now derive $M$, the number of reduced samples needed to verify cruel bit guesses, and consequently the amount of pre-processing resources needed for our attack. Since in practice the distribution of residuals is indistinguishable from uniform over $[0,q]$ when the cruel bits are incorrectly chosen, we frame the task of identifying correct cruel bits as distinguishing from uniform. As describe in Section \ref{sec:practical}, we do so by measuring the variance.
First, we calculate $\hat{\sigma}^2(x)$ over $M$ reduced samples via
\begin{align}
\hat{\sigma}^2 = \frac{1}{M}\sum_{i=0}^{M-1}x_i^2.
\end{align}
We can construct a lower confidence bound $\iota$ for the variance under the null hypothesis of uniformity, assuming a Gaussian distribution of $\hat{\sigma}^2$ under the CLT:
\begin{align}
\iota(\alpha, M) = \sigma_{\mathcal{U}_q}^2 + G^{-1}(\alpha) \cdot \sqrt{\frac{\sigma^2_{\mathcal{U}_q^2}}{M}} =  \sigma_{\mathcal{U}_q}^2 + G^{-1}(\alpha) \cdot \sqrt{\frac{\sigma_{\mathcal{U}_q}^2}{M} \cdot \frac{q^2-4}{15}},
\end{align}
where $G^{-1}$ is the percent point function of $\mathcal{N}(0,1)$ and $\sigma_{\mathcal{U}_q}^2$ (resp. $\sigma^2_{\mathcal{U}_q^2}$) is the distribution variance of $x$ (resp. $x^2$) under the null hypothesis of uniformity. $\alpha$ is the type-I error, i.e. the probability of rejecting a true null hypothesis. Since we are brute-forcing a large number of possible solutions, the type-I error, $\alpha$ should be small (i.e. $\alpha <$ the inverse of the number of secret candidates).

Given $\alpha$ and $\beta$ type-II error (the probability of failing to reject a false null hypothesis), we can estimate the minimum number of samples needed for our attack to succeed with probability $\approx 1-\beta$ using CLT (see \ref{sec:m_formula_dx} for more details): 
\begin{align}
 \label{eq:Msamples}
 M(\alpha, \beta) =  \Biggl [\frac{ G^{-1}(\alpha) \sigma_{\mathcal{U}_q^2} + G^{-1}(\beta)\sigma_{\mathcal{G}_q^2}}{(\sigma^2_{\mathcal{G}_q} - \sigma^2_{\mathcal{U}_q})} \Biggr ]^2 
\end{align}
where $ \sigma_{\mathcal{G}_q}$ resp. $ \sigma_{\mathcal{G}_q^2}$ is the standard deviation of 
$x$ resp. $x^2$ when $x\sim \mathcal{G}_q$ i.e. discrete centered Gaussian mod $q$. Table~\ref{tab:datasummary} gives concrete calculations of $M$ for various $h$ secrets.


\begin{table}[h]
\vspace{-0.5cm}
    \small
    \centering
    \caption{\small Number of samples $M$ needed in the statistical test for type-I error $\alpha = 2^{-128}$ and type-II error $\beta = 10^{-5}$ for LWE settings specified by $n$, $\log_2 q$, $n_u$, and secret Hamming weight $h$. The Worst Case number of samples corresponds to the case where all the 1s in the secret are in the reduced region $h_r = h$, whereas the Average case assumes the average number of 1s in that region, which is the fraction $\frac{n_r}{n}h$} 
    %\kl{what is the last column showing? can we just write 0.145? Also $n_r = n - n_u.$}
    
    \vspace{0.1cm}
    \label{tab:datasummary}
    \setlength{\tabcolsep}{5pt}
    \begin{tabular}{cccccc}
    \toprule
     $n$ & $\log_2 q$ & $n_u$ & $h$ & Worst case $M$ & Average case $M$ \\ %& Average Case \\
     & & & &$(h_r = h)$ &$(h_r = \frac{n_r}{n}h)$ \\ %& $(\sigma^2_{\mathcal{U}_q}-\sigma^2_{\mathcal{G}_q})/\sigma^2_{\mathcal{U}_q}$\\
    \midrule
    256 & 12 & 143 & 12 & $5.67\times 10^{4}$ & $1.12\times 10^{4}$ \\ %& $1.45\times 10^{-1}$ \\
512 & 28 & 228 & 20 & $3.29\times 10^{3}$ & $1.66\times 10^{3}$ \\ %& $3.64\times 10^{-1}$ \\
512 & 41 & 75 & 60 & $1.98\times 10^{4}$ & $1.02\times 10^{4}$ \\ %& $1.51\times 10^{-1}$ \\
768 & 35 & 373 & 20 & $3.13\times 10^{4}$ & $9.74\times 10^{3}$ \\ % & $1.55\times 10^{-1}$ \\
768 & 35 & 373 & 64 & $6.21\times 10^{6}$ & $1.47\times 10^{5}$ \\ %& $4.03\times 10^{-2}$ \\
    \bottomrule
    \end{tabular}
    \vspace{-0.2cm}
\end{table}

These results indicate that in the easiest settings (e.g. $n=512$) a few thousand reduced samples are enough to test cruel bit guesses. For $n=256$, a few tens of thousands of reduced pairs are needed.
As indicated in Section \ref{sec:practical}, the amount of data used can be traded off by running the cool bit estimation and subsequent secret check more often.

%\para{Empirical data estimation.} For clarity, we empirically explore the number of samples needed for cruel bit recovery, leveraging our knowledge of true secret $\mathbf{s}$. For given values of $h_r$ and $h_u$, we generate a set of candidate secrets $\mathbf s^*$, and compute for each $\mathbf s^*$, \kl{and for the secret $\mathbf s$,}% (how? if we don't have s?)},
%the standard deviation $\sigma(x)$, over a set of previously reduced pairs $(\mathbf a,b)$. 
 
% Figure~\ref{fig:empirical_secret} shows the distributions of $\sigma(x)$ for $n=768$, $\log q=35$, $h=64$, generated by calculating $\sigma(x)$ with varying $M$ (10K, 50K, and 200K) and 50K candidate secrets. The standard deviation for a secret with correct cruel bits, $\sigma_t$, is shown in red. 
%  With the exception of the true secret outlier $\sigma_t$, $\sigma(x)$ follows a Gaussian distribution centered at $q/\sqrt{12}$ as expected. As the number of $(\mathbf{a}, b)$ pairs grows, $\sigma_t$ becomes more easily distinguishable from the rest of the distribution. We observe that $M$ needed in practice is smaller than our estimates, because our theory assumes a much smaller $\alpha$ than is needed in practice. % \todo{Need to nuance this discussion since it seems we empirically need much less data than we estimate. NN: is that actually true?}

% \begin{figure*}[h]
% \begin{center}
%     \subfigure[$10$K ($\mathbf{a}, b$) pairs]{\includegraphics[width=0.31\linewidth]{figs/dist_n768_logq35_10000.pdf} }
%     \subfigure[$50$K ($\mathbf{a}, b$) pairs]{\includegraphics[width=0.31\linewidth]{figs/dist_n768_logq35_50000.pdf} }
%     \subfigure[$200$K ($\mathbf{a}, b$) pairs]{\includegraphics[width=0.31\linewidth]{figs/dist_n768_logq35_200000.pdf} }
% \end{center}
% \vspace{-0.6cm}
% \caption{Empirical $\sigma(x)$ distribution for $n=768$, $\log q=35$, $h=64$ computed with $50K$ candidate secrets and different $M$. The $\sigma(x)$ of true secret $\mathbf{s}$ is indicated by the red line.} %\kl{what is the red vertical line?}
% \label{fig:empirical_secret}
% \end{figure*}

\vspace{-0.5cm}

\subsection{Testing cool bit predictions.}\label{sec:cool_bits}

Once the cruel bits have been guessed, we can use Algorithm~\ref{alg:greedy_cool} to recover the cool bits of the secret one bit at a time. As before, we will estimate the standard deviation of $x=\mathbf a \cdot \mathbf s^* - b$ over a sample of reduced LWE pairs, but the cruel bits in our guess $\mathbf s^*$ are now assumed to be correct. For each cool coordinate, we compare the secret $\mathbf s$ with two guesses $\mathbf s_0^*$, and $\mathbf s_1^*$ which agree with the secret on the $k-1$ first characters, are zero on the $n-k$ characters, and have their $k$-th bit set to $0$ and $1$ respectively. If the $k$-th bit is zero, $x_0=\mathbf a\cdot \mathbf s_0^* - b$ should have a lower standard deviation than $x_1=\mathbf a\cdot \mathbf s_1^* - b$. 

Suppose that all the cruel bits and the $k-1$ first cool coordinates have been correctly guessed, and there are $h^*$ one bits to be discovered in the remaining cool coordinates. Let the null hypothesis be $H_0: \mathbf s_k = 0$ and the alternative hypothesis: $H_1: \mathbf s_k = 1$. The residual $x_0=\mathbf a\cdot \mathbf s_0^* - b$ has in both cases variance 
%\begin{align}
$\sigma^2_0=F_q(h^*\sigma_r^2+\sigma_e^2)$.
%\end{align}
Under $H_0$ the variance of $x_1=\mathbf a\cdot \mathbf s_1^* - b$ will be
%\begin{align}
$\sigma^2_{+1}=F_q((h^*+1)\sigma_r^2+\sigma_e^2) > \sigma^2_0$.
%\end{align}
Under $H_1$ the variance of $x_1$ is 
%\begin{align}
$\sigma^2_{-1}=F_q((h^*-1)\sigma_r^2+\sigma_e^2) < \sigma^2_0$.
%\end{align}

In each iteration $k$ of \cref{alg:greedy_cool}, our objective is to determine whether the difference in estimated variance, denoted as $\delta (\sigma^2) := \hat{\sigma}^2(x_{1}) - \hat{\sigma}^2(x_0)$, is more closely aligned with $\sigma^2_{+1} - \sigma^2_0 > 0$ or $\sigma^2_{-1} - \sigma^2_{0} < 0$. To achieve this, we estimate the variance difference using enough samples. Without the need for optimal threshold tuning, we reject the null hypothesis if the variance difference $\delta(\sigma^2)$ is negative, and accept it otherwise.

%Table~\ref{tab:coolrecovery} gives the ratios of standard deviations for different $k$ and problem settings. The standard deviation difference between correct and incorrect predictions is much smaller than the difference when guessing cruel bits. However, we can also afford a larger error rate here, because scaling is linear with $n_r$.
%
%\begin{table}[h]
%\vspace{-0.5cm}
%    \small
%    \centering
%    \caption{\small \textbf{Cool bit recovery.} Ratio of standard deviations, $\sigma(x_{k})/\sigma(x_{k+1})$, varying $k$.}
%    \vspace{0.1cm}
%    \label{tab:coolrecovery}
%    \begin{tabular}{cc@{\hskip 12pt}ccccc}
%        \toprule
%        & & \multicolumn{5}{c}{$\sigma(x_{k})/\sigma(x_{k+1})$} \\
%        \cmidrule(lr){3-7}
%        n& $\log_2 q$ & $k=3$ & $k=5$ & $k=10$ & $k=15$ & $k=20$ \\
%        \midrule
%        256 & 12 & 0.989 & 0.990 & 0.995 & 0.998 & 0.998 \\
%        512 & 28 & 0.984 & 0.986 & 0.988 & 0.990 & 0.993 \\
%        512 & 41 & X & X & X & X & X \\
%        768 & 35 & 0.992 & 0.993 & 0.994 & 0.996 & 0.997 \\
%       \bottomrule
%    \end{tabular}
%    \vspace{-0.3cm}
%\end{table}
%\kl{need to fill in the Xs}

%Because the difference  

%Let $s^*$ be our secret estimate, $\mathbf s$ the secret, $\mathbf  A$ the matrix of $N$ reduced vectors $\mathbf a$, and $\mathbf b=\mathbf A \cdot \mathbf s + e$. 

%(with $n_a$ the number of annoying bits). Both tests rely on comparing the standard deviations of $\mathbf A \cdot \mathbf s^* - \mathbf b = \mathbf A \cdot (\mathbf s^* - \mathbf s) + e$ if $\mathbf s^*$ is ``correct'' and if $\mathbf s^*$ is wrong. 

%Let $n_a$ be the number of annoying bits, $A_a$ the restriction

%\subsection{Testing secret guesses.}
%
%Secret guesses $\mathbf s^*$ can be tested from LWE pairs $(\mathbf a,b)$ by computing the standard deviation of $x=\mathbf a \cdot \mathbf s^* - b$. If the prediction is correct ($\mathbf s^*=\mathbf s$), $\sigma(x)$ should be very close to the error (a small number). If it is incorrect, it should be close to  $\frac{q}{\sqrt{12}}$.
%This test is very accurate~\cite{picante}. Table~\ref{tab:testguess} provides confidence intervals for tests using $n$ and $4n$ pairs, for different problem sizes.
%Given the extreme accuracy and efficiency of that check, we omit it in practice and simply compare against the true secret directly.
%
%\begin{table}[h]
%    \small
%    \centering
%    \caption{\small \textbf{Testing guessed secrets.} Confidence intervals ($\alpha=0.001$) of standard deviation of $x$, for correct and incorrect guesses.}
%    \label{tab:testguess}
%    \begin{tabular}{
%        cc
%        @{\hskip 12pt}
%        cc
%        @{\hskip 12pt}
%        cc
%    }
%        \toprule
%        & & \multicolumn{2}{c}{4n LWE samples} & \multicolumn{2}{c}{n LWE samples} \\
%        \cmidrule(lr){3-4} \cmidrule(lr){5-6}
%        $n$ & $\log_2 q$ & Correct & Incorrect & Correct & Incorrect \\
%        \midrule
%        256 & 12 & [2.8, 3.3] & [897.9, 1039.6] & [2.6, 3.6] & [845.8, 1141.2]\\
%        512 & 28 & [2.9, 3.2] & [$4.9\cdot 10^7$, $5.5\cdot 10^7$] & [2.7, 3.4] & [$4.7\cdot 10^7$, $5.8\cdot 10^7$] \\
%        768 & 35 & [2.9, 3.1] & [$9.4\cdot 10^9$, $1.03\cdot 10^{10}$] & [2.8, 3.3] & [$9.1\cdot 10^9$, $1.08\cdot 10^{10}$] \\
%       \bottomrule
%    \end{tabular}
%%    \vspace{-0.5cm}
%\end{table}

%\subsection{Number of samples needed for cruel bit discovery}

%Analysis of the empirical distribution of standard deviations}
% Emily's rough draft.


%crrect and the $x_{true} = \mathbf{a \cdot s_{true}} - b$ is shown in red. 

% \begin{figure*}[t]
% \begin{center}
%     \begin{minipage}[c]{0.32\linewidth}
%         \includegraphics[width=1.0\textwidth]{figs/fitted_n256_logq12.pdf}
%         \vspace{-0.5cm}
%         \caption{Fitted Gaussian for $n=256$, $\log q=12$, $h=16$.}
%         \label{fig:fitted1}
%     \end{minipage}\hfill %
%  \begin{minipage}[c]{0.32\linewidth}
%         \includegraphics[width=1.0\textwidth]{figs/fitted_n256_logq20.pdf}
%         \vspace{-0.5cm}
%         \caption{$n=256$, $\log q=20$, $h=40$.}
%         \label{fig:fitted2}
%     \end{minipage}\hfill%
% \begin{minipage}[c]{0.33\linewidth}
%         \includegraphics[width=1.0\textwidth]{figs/fitted_n1024_logq50.pdf}
%         \vspace{-0.5cm}
%         \caption{$n=1024$, $\log q=50$, $h=64$.}
%         \label{fig:fitted3}
%     \end{minipage}
% \end{center}
% \end{figure*}


 % To find the probability of an incorrect secret producing an $\sigma(x) \le \sigma_t$, we fit a Gaussian distribution to the empirical distribution of $\sigma(x)$ and compute the CDF. Figures~\ref{fig:fitted1}-\ref{fig:fitted3} provide examples of such fitted Gaussians.
% \begin{table}[h]
%     \centering
%     \small
%     \caption{Example fitted Gaussian distributions to $\sigma(x)$ values for varying $n/\log q$, along with $\sigma_t$ values, and the probability of $\sigma(x) \le \sigma_t$}
%     \begin{tabular}{cccccc}
%     \toprule
%         n & $\log q $ &  $h$ & $\sigma(x) \sim \mathcal{N}(\mu, \sigma)$ & $\sigma_t $ (correct cruel bits) & $ \text{CDF}(\sigma_t)$   \\ \midrule
%         256  & 12 & 16 & $\mathcal{N}(961, 4.7)$ & 940 &  $6.0\cdot 10^{-6}$ \\
%         256  & 20 & 40 & $\mathcal{N}(2.4\cdot10^5, 343)$ & 241105 &  $9.8\cdot 10^{-11}$ \\ 
%         1024  & 50 & 64 & $\mathcal{N}(1.75 \cdot 10^{14}, 3.5\cdot10^{11})$ & $1.74\cdot 10^{14}$  & $9\cdot 10^{-4}$ \\ 
%         \bottomrule
%     \end{tabular}
%     \label{tab:stdev_results}
% \end{table}
% We compute the probability of $\sigma(x) \le \sigma_t$ via the CDF. These results are shown in Table~\ref{tab:stdev_results}.

% \begin{figure}[t]
%     \centering
% \includegraphics[width=0.45\textwidth]{figs/prob_vs_data.pdf}
%     \caption{Number of $(\mathbf{a}, b)$ pairs used to fit $x$ distribution vs. the CDF$(\sigma_t)$ in log-scale for $n=256$, $\log q = 12$, $h=16$.}
%     \label{fig:prob_vs_data}
% \end{figure}

% We also consider how the number of $(\mathbf{a}, b)$ pairs used to compute $\sigma(x)$ affects the statistical significance of the comparison with $\sigma_t$. Figure~\ref{fig:prob_vs_data} shows the CDF value as a function of number of samples used for the test. For this particular case of $n=256$, $\log_2 q=12$, $h=16$, $5000$ pairs are needed. 


==> AFRICACRYPT_SUBMISSION/header.tex <==

\usepackage{microtype}
\usepackage{graphicx}
\usepackage{subfigure}
\usepackage{booktabs} 
\usepackage{multirow}

\usepackage{hyperref}
\usepackage{caption}
\usepackage{xcolor}
\usepackage{color}

\usepackage{amsmath,amssymb,amscd,url,enumerate, mathtools}
\usepackage[utf8]{inputenc}
\usepackage{wrapfig}
\usepackage{pdflscape}
\usepackage{tikz}
\usetikzlibrary{decorations.markings,arrows}
\usetikzlibrary{positioning,arrows,fit}
\renewcommand\vec[1]{\boldsymbol{#1}}
\usepackage{tikz-cd}
\usepackage{amsfonts}
\usepackage{amsmath}
\usepackage{graphicx}
%\usepackage{amsthm}
\usepackage{mathrsfs}
\usepackage{dsfont}
\usepackage{enumitem}
\usepackage{array}
\usepackage{verbatim}
\usepackage{ulem}
\newcolumntype{?}{!{\vrule width 1pt}}
\usepackage[capitalize,noabbrev]{cleveref}
\usepackage[font=footnotesize,labelfont=bf, labelsep=period, textfont=sl]{caption}
%\usepackage{algorithmic}
%\usepackage{algorithm}

\newcommand{\largedot}{\resizebox{0.3em}{!}{\ensuremath{\bullet}}}



\newcommand{\para}[1]{{\vspace{2pt} \bf \noindent #1}}  
\newenvironment{packed_itemize}{
\begin{list}{\labelitemi}{\leftmargin=1em}
\setlength{\itemsep}{1pt}                                                           
\setlength{\parskip}{0pt}                                                                                 \setlength{\parsep}{0pt}                                                                                  \setlength{\headsep}{0pt}                                                                                 \setlength{\topskip}{0pt}                                                                                 \setlength{\topmargin}{0pt}                                                                               \setlength{\topsep}{0pt}                                                                                  \setlength{\partopsep}{0pt}                                                                               }{\end{list}}                                                                                                                                  

\newenvironment{packed_enumerate}{  
\begin{enumerate}                                                                                         \setlength{\itemsep}{3pt}                                                                                 \setlength{\parskip}{0pt}                                                                                 \setlength{\parsep}{0pt}                                                                                  \setlength{\headsep}{0pt}                                                                                 \setlength{\topskip}{0pt}                                                                                 \setlength{\topmargin}{0pt}                                                                               \setlength{\topsep}{0pt}                                                                                  \setlength{\partopsep}{0pt}
}{\end{enumerate}} 

\newcommand{\ZZ}{\mathbb{Z}}

\DeclarePairedDelimiter\floor{\lfloor}{\rfloor}
\DeclarePairedDelimiter\ceil{\lceil}{\rceil}

% for adjustwidth environment
\usepackage[strict]{changepage}

% for formal definitions
\usepackage{framed}

% environment derived from framed.sty: see leftbar environment definition
\definecolor{formalshade}{rgb}{0.95,0.95,1}

\newenvironment{formal}{%
  \def\FrameCommand{%
    \hspace{1pt}%
    {\color{blue}\vrule width 2pt}%
    {\color{formalshade}\vrule width 4pt}%
    \colorbox{formalshade}%
  }%
  \MakeFramed{\advance\hsize-\width\FrameRestore}%
  \noindent\hspace{-4.55pt}% disable indenting first paragraph
  \begin{adjustwidth}{}{7pt}%
  \vspace{2pt}\vspace{2pt}%
}
{%
  \vspace{2pt}\end{adjustwidth}\endMakeFramed%
}
%%%%%% CUSTOM COMMANDS %%%%
%
\newcommand{\T}{\mathcal{M}}
% 
\newcommand{\system}{{\textsc{Verde}}}
\newcommand{\salsys}{{\textsc{Salsa} \textsc{Verde}}}
\newcommand{\salsa}{{\textsc{Salsa}}}
\newcommand{\picante}{{\textsc{Picante}}}
\newcommand{\tinyLWE}{{\textsc{TinyLWE}}}
\newcommand{\lwe}{\textsc{lwe}}
\newcommand{\fplll}{{\textit{fplll}}}
\newcommand{\nomod}{{\textbf{NoMod}}}
\newcommand{\std}[1]{{\text{stddev}\left({#1}\right)}}
\newcommand{\var}[1]{{\text{Var}\left({#1}\right)}}


\definecolor{lightgreen}{HTML}{117733}
\definecolor{lred}{HTML}{FF0000}
\newcommand{\success}[1]{\textcolor{lightgreen}{\textbf{#1}}}
\newcommand{\fail}[1]{\textcolor{lred}{{\em #1}}}
\newcommand{\todo}[1]{\textcolor{red}{{TODO: {\em #1}}}}

\newcommand{\nolte}[1]{\textcolor{brown}{[NN] #1}}
\newcommand{\kl}[1]{\textcolor{purple}{[KL] #1}}
\newcommand{\fc}[1]{\textcolor{orange}{[FC] #1}}
\newcommand{\emily}[1]{\textcolor{lightgreen}{[EW] #1}}
\newcommand{\mm}[1]{\textcolor{teal}{[MM] #1}}


==> AFRICACRYPT_SUBMISSION/intro.tex <==
\section{Introduction}
\label{sec:intro}



%% PARA 1: Sparse secrets are a thing
Lattice-based cryptosystems are attractive candidates for Post-Quantum Cryptography (PQC), standardized by NIST in the 5-year PQC competition (2017-2022) and by the Homomorphic Encryption community~\cite{HES,nist2022finalists}.   
Special parameter choices, such as binary, ternary, binomial, or Gaussian secrets, small error, or small {\it sparse} secrets, are often made to improve efficiency or functionality.
Homomorphic Encryption (HE) implementations routinely assume small error and sparse binary or ternary secrets~\cite{HES,params_heean}, and the NIST-standardized Kyber schemes assume small secret and small error (binomial distribution)~\cite{nist2022finalists}.  


Although these implementation choices may weaken security of the lattice-based cryptosystems, surprisingly few concrete results and benchmarks exist to quantify the actual time and resources required to attack systems with sparse secrets and small error. 
Over the last few decades, the lattice cryptography community has developed theoretical predictions of time and resources needed to attack lattice-based cryptosystems in general by studying and improving lattice reduction algorithms, such as LLL, BKZ, BKZ2.0 with various strategies such as sieving, early abort etc. (\cite{LLL,CN11_BKZ,fplll}). 
To estimate the performance of these algorithms, the community relies on the LWE Estimator~\cite{LWEestimator}, but these estimates are often inaccurate for special parameter choices and for parameter sizes that can be tested in practice. 
While some attacks on sparse secrets have been proposed, such as the Sparse dual attack~\cite{Albrecht2017_sparse_binary} and the Hybrid Sparse Dual Meet-in-the-Middle attack~\cite{Cheon_hybrid_dual}, general benchmarks for measuring attacks on small sparse secrets have not yet been developed. Existing benchmarks, such as the Darmstadt Lattice Challenges~\cite{darmstadt_lwe} are not relevant, since they do not cover such parameter choices.
%So more work is needed to assess the hardness of sparse binary secrets in practice, and to develop concrete benchmarks. 

\para{Our Contribution.} Given the potentially widespread adoption of lattice cryptosystems with sparse, small secrets, more work is needed to assess their hardness.  
To that end, we provide a new tool for attacking sparse small secrets, based on the observation that lattice reduction with certain parameters separates secrets into ``cruel bits'', corresponding to unreduced data which is hard to analyze, and ``cool bits'' that can be recovered in linear time once the hard bits are known. This leads us to define an attack on sparse small secrets, in three stages:

%and profile the resulting attack which applies especially well to sparse binary secrets. The new tool is the observation that we can separate out the hard bits of the secret (the ``cruel bits'') after some partial lattice reduction, and then we can recover the rest of the easier ``cool'' bits in linear time.
%
%More precisely, the current paper presents a new observation about hard bits after partial lattice reduction, and a statistical attack which relies on it. The attack stages are:

\begin{enumerate}
\item initial partial lattice reduction in parallel; 
\item brute force recovery of a small number of hard, cruel bits; 
\item statistical recovery of cool bits, and the secret.
\end{enumerate}
We provide concrete experimental results for our attack, demonstrating its efficacy on LWE instances with sparse binary secrets in dimension $n \le 768$. Furthermore, we show how this attack applies to both LWE and RLWE instances, with RLWE instances being much more vulnerable. We believe this attack should be taken into account whenever sparse secrets are being proposed, since a significant fraction of secrets are vulnerable to it (see Table~\ref{tab:experiments_recovery}), and we hope it provides a helpful practical benchmark for future research.  
% For example, see Table~\ref{tab:experiments_recovery} for surprisingly quick secret recoveries for a given Hamming weight.
% \sam{Remove this sentence after I add the highlight table.}
% \fc{Do we want to try to quantify this likelihood?}

\para{High-Level Attack Idea.} Our key observation is that, for an LWE instance $(\mathbf{A}\in \mathbb{Z}_q^{m \times n}, b \in \mathbb{Z}_q^m)$, lattice reduction of q-ary embedded matrices of the form 
\begin{align}
\mathbf \Lambda = 
\begin{pmatrix}
0 & q \mathbf{I}_n \\
\omega \mathbf{I}_m &\mathbf  A
\end{pmatrix},
\end{align}
produces a reduced matrix $\mathbf A'$ with a non-uniform distribution of variances over its columns%of the reduced matrix $\mathbf{A}$ matrix extracted from the lattice embedding post-reduction
, see \cref{sec:attack} for details. Specifically, the variance of the first $n_u$ columns of $\mathbf A'$ is unaffected by lattice reduction. We call the bits of the secret in the first $n_u$ columns ``cruel" (unreduced). The other $n_r = n - n_u$ columns of the matrix have significantly reduced variance, and we call the secret bits corresponding to these columns the ``cool" bits. The number of unreduced and reduced columns of $\mathbf{A}'$, $n_u$ and $n_r$, depends on the overall lattice reduction quality and the penalty parameter $\omega$, which controls a trade-off between reduction and the error variance after reduction.

Our attack leverages this observation to reduce the original LWE problem to one with higher error on only the “cruel” entries in $\bf{A}$, by essentially ignoring the ``cool" bits. If the error introduced by the ignored bits is sufficiently small, a secret guess $s^*$ where only the first $n_u$ bits are correct can be identified with sufficient statistics.
The remaining (cool) bits can then be recovered one by one.
%Table \ref{tab:highlights} shows successful secret recovery attacks on the LWE problem using our proposed attack.  See Table \ref{tab:experiments_recovery} for additional results.
% \begin{table}[h]

% \vspace{-0.6cm}
%     \centering
%     \small
%     %\resizebox{0.5\textwidth}{!}{
%     \caption{
%         Successful LWE secret recovery attacks leveraging our cruel/cool observation for various $n$/$q$ and Hamming weight $h$ settings. The timings do not include time for parallelized lattice reduction.}
%         \vspace{0.1cm}
%             \label{tab:highlights}
%     \begin{tabular}{
%         c
%         @{\hskip 6pt}
%         S[table-format=2.0]
%         @{\hskip 6pt}
%         S[table-format=2.0]
%         @{\hskip 6pt}
%         S[table-format=4.0]
%     }

%         \multicolumn{4}{c}{LWE Results} \\
%                 \toprule
%         {$n$} & {$\log_2 q$} & {$h$} & {Time (Sec)} \\
%         \midrule
%         \multirow{1}{*}{256} & 12 & 12 & {$4.81\times 10^7$} \\
%       %  & 20 & 40 & 57 \\
%         \cmidrule(lr){2-4}
%         \multirow{2}{*}{\num{512}} & 28 & 12 & {$9.65\times 10^6$}\\
%         & 41 & 60 & {$1.02\times 10^9$} \\
%         \cmidrule(lr){2-4}
%         \num{768} & 35 & 12 & {$3.59\times 10^7$} \\
%         \bottomrule
%     \end{tabular}\hspace{0.5cm}%\hfill
%     %}\
%        \begin{tabular}{
%         c
%         @{\hskip 6pt}
%         S[table-format=2.0]
%         @{\hskip 6pt}
%         S[table-format=2.0]
%         @{\hskip 6pt}
%         S[table-format=4.0]
%     }

%         \multicolumn{4}{c}{RLWE Results} \\
%                 \toprule
%         {$n$} & {$\log_2 q$} & {$h$} & {Time (Sec)} \\
%         \midrule
%         \multirow{1}{*}{256} & 12 & 12 & {$4.08\times 10^4$} \\
%       %  & 20 & 40 & 57 \\
%         \cmidrule(lr){2-4}
%         \multirow{2}{*}{\num{512}} & 28 & 12 & {$2.03\times 10^4$} \\
%         & 41 & 60 & {$2.01\times 10^5$} \\
%         \cmidrule(lr){2-4}
%         \num{768} & 35 & 12 & {$1.42\times 10^5$} \\
%         \bottomrule
%     \end{tabular}
%        % \caption{Caption}
%        % \label{tab:my_label}
% \end{table}
\begin{table}[h]
\vspace{-0.85cm}
    \centering
    \small
    \caption{
        Successful LWE secret recovery attacks leveraging our cruel/cool observation for various $n$/$q$ settings. The timings do not include time for parallelized lattice reduction.}
        \vspace{0.1cm}
    \begin{tabular}{
        c
        @{\hskip 6pt}
        S[table-format=2.0]
        @{\hskip 6pt}
        S[table-format=2.0]
        @{\hskip 6pt}
        S[table-format=4.0]
    }
        \toprule
        $n$ & {$\log_2 q$} & {Hamming Weight} & {Time (Sec)} \\
        \midrule
        \multirow{2}{*}{256} & 12 & 12 & 3865 \\
      %  & 20 & 40 & 57 \\
        \cmidrule(lr){2-4}
        \multirow{2}{*}{\num{512}} & 28 & 12 & 2417\\
        & 41 & 60 & 376 \\
        \cmidrule(lr){2-4}
        \num{768} & 35 & 12 & 1291 \\
        \bottomrule
    \end{tabular}
    \label{tab:highlights}
    \vspace{-0.5cm}
\end{table}

\cref{tab:highlights} presents parameter settings and timings for successful recovery of sparse binary secrets, and demonstrates the benefits of cruel-cool bit separation in non-trivial LWE settings (see~\cref{tab:experiments_recovery} for additional results).
In these examples, Hamming weights were selected so that secret recovery from reduced matrices only takes a small amount of compute. We choose those settings because the lattice reduction step is theoretically least well understood, whereas the rest of the attack can be understood better theoretically (see \cref{sec:theory}) and does not need extensive experimentation.
For example, for dimension $n=512$ and $\log_2 q =41$, our attack recovers binary secrets with Hamming weight $60$ in about $6$ minutes on one GPU.  This does not include the time spent on lattice reduction to prepare the data, which is about $12$ hours/matrix (see Table~\ref{tab:datasets}).  
Table~\ref{tab:highlights} also shows successful secret recovery for larger dimensions, such as $n=768$ and $\log_2 q =35$, for binary secrets with Hamming weight $12$, in roughly $22$ minutes using $20$ GPUs.

\para {RLWE attack.} Our attack can also be applied in the Ring-LWE setting.  When the ring is a $2$-power cyclotomic ring defined by the polynomial $x^n+1$, where $n=2^k$, then the RLWE samples corresponding to a polynomial RLWE sample, $(a(x), b(x) = a(x) \cdot s(x) + e(x))$ can be described via a skew-circulant matrix, $A_{circ}$; see Section~\ref{sec:RLWE} for details. When the matrix has this structure, we can rotate the ``cruel bits'' around (without redoing any lattice reduction) by inspecting samples from only certain indices of circulant matrices. This greatly increases our chances of recovering the secret and makes attacking the 2-power cyclotomic RLWE problem clearly easier than generic LWE.  We give concrete timings for the RLWE setting, estimate the average speed-up over LWE, and show the improved success rate in~\cref{sec:RLWE}.



%
%\begin{table}[h]
%    \centering
%    \small
%    \begin{tabular}{S[table-format=3.0]cccc}
%        \toprule
%        {$n$} & $\log_2 q$ & $h$ & Compute & Mean Time \\
%        \midrule
%        256 & 12 & & \multirow{3}{*}{256 XXX CPU, 4x V100} \\
%        512 & 28 & & \\
%        768 & 35 & & \\
%        \bottomrule
%    \end{tabular}
%    \caption{
%        Best recovered secrets across several values of $n$.
%        \sam{quick highlights table}
%    }
%    \label{tab:highlights}
%\end{table}

\para{Outline of the paper.} \cref{sec:compare} describes related work. \cref{sec:attack} presents our attack in detail. \cref{sec:reduction} explains the lattice reduction step for processing LWE samples to use in the attack. \cref{sec:theory} contains the statistical analysis of the attack, including an estimate for number of samples needed. \cref{sec:results} presents our concrete secret recovery results and displays performance of other attacks. 
\cref{sec:RLWE} adapts the attack to the RLWE setting and shows the improvement there. See \href{https://github.com/anonymous}{[redacted link]} for the Python code for running the attack. 


==> AFRICACRYPT_SUBMISSION/overview.tex <==
\section{High-level summary of SALSA's current state}
\label{sec:overview}

% ******deprecated******  TO BE MOVED elsewhere, or partially included in intro: 


% Since the submission of Verde to NeurIPS in mid-May 2023, significant progress has been made along several axes. Preprocessing has been drastically improved, both by reducing compute resource requirements, 
% % cathy: the storage improvement is for experiments when we share the same reduced A. Doesn't help in the wild. 
% as well as by integrating Flatter~\cite{ryan2023fast}, a fast lattice reduction algorithm leveraging iterated compression. Reductions that used to take $\approx 35$ days now take less than $2$. We have also explored the use of novel model architectures. The seq2seq model used in the prior three SALSA papers has been replaced by a smaller, encoder-only transformer, which runs a little faster, takes up less memory, and has more fine-grained probability outputs which can make secret recovery easier. Additional exploration of pretraining/curriculum learning. novel embedding techniques, and other new training methods is underway. Finally, we have expanded the types of secrets we can recover via the addition of a binomial distinguisher. This distinguisher, which expands upon some of the ideas in the original ternary secret distinguisher, allows recovery of secrets with coordinates in $[-2, 2]$. 

% Together, these advances have moved the SALSA attack to the point where it {\em may} outperform all other SOTA attacks on lattices of its size. Scaling trends are still not well-understood, but with the theory results from Verde they may be easier to generate now. Therefore, the goals of this writeup are threefold: {\bf to summarize progress made in summer 2023}, to {\bf provide a snapshot of our attack's performance vs. other SOTA attacks}, and to {\bf outline a plan for future work}. 


Copying Francois's statistical analysis here:

\subsection{Statistical calculation of sample size}

During the attack, three statistical tests must be performed: 
\begin{itemize}[nosep]
\item when enumerating the cruel bits, to decide if this is a likely solution 
\item when enumerating the cool bits (for one set of cruel bits), to decide if a bit is zero or one 
\item when a secret candidate was found, to test it.
\end{itemize}

For the last test, we use the technique described in SALSA PICANTE~\cite{}. Given a set of $p$ LWE pairs $(\mathbf a,b)$, for a secret prediction $\mathbf s^*$, we compute the standard deviation of $x=\mathbf a \cdot \mathbf s^* - b$, which should be close to the error (i.e. very small) if $\mathbf s^*$ is the correct secret, and close to $\frac{q}{\sqrt{12}}$ if it is not. This test is very accurate, even for small values of $p$ (e.g. $p=n$, see Table~\ref{}).

\paragraph{Testing cruel bit predictions.} This test is performed every time we guess the cruel bits. Let $\mathbf s^*$ be the secret estimate built by setting all cruel bits to their current predictions, and all cool bits to zero. Suppose we have a set of $m$ reduced LWE samples $(\mathbf a,b)$ for the secret $\mathbf s$, with error $e$ and reduction factor $\rho$. Consider the random variable $x = \mathbf a \cdot \mathbf s^* - b = \mathbf a \cdot (\mathbf s^* - \mathbf s)-e \mod q$. Our intuition is that the standard deviation of $x$ will be lower when all cruel bits are correctly predicted. By estimating it on a large enough sample of reduced pairs (i.e. with $m$ large enough), we can build a reliable test. Our goal, here, is to provide a theoretical estimate of $m$.

More precisely, let $n$ and $h$ be the problem dimension and secret Hamming weight considered. Let $n_\text{cruel}$ be the number of cruel bits, and $h_\text{cruel}$ the Hamming weight of the cruel bits. On the reduced LWE samples, the $n_\text{cruel}$ first coordinates of $\mathbf a$, which correspond to the cruel bits, have a standard deviation $\sigma_u=q/\sqrt{12}$ (the standard deviation of a uniform distribution over $[0,q)$), let $\sigma_c$ be the standard deviation of the $n-n_\text{cruel}$ next coordinates (the cool coordinates). Assuming that all reduced coordinates of $\mathbf a$ are independent (this is a worst case CHECK IF IT HOLDS IN PRACTICE!!), we have $$\rho^2 \sigma_u^2 = \frac{n_\text{cruel}}{n} \sigma_u^2+\frac{n-n_\text{cruel}}{n}\sigma_c^2,$$
and therefore %$$\sigma_c^2 = \frac{\rho^2 n - n_a}{n-n_a} \sigma_u^2,$$
$$\sigma_c = \sqrt{\frac{\rho^2 n - n_\text{cruel}}{n-n_\text{cruel}}} \sigma_u.$$

Using the examples in table~\ref{tab:data}, for $n=256$ and $\log_2 q=12$, we have $\rho=0.749$, $n_\text{cruel}=137$ and $\sigma_c=0.24 \sigma_u$. For $n=512$ and $\log_2 q=24$ we have $\rho=0.722$, $n_\text{cruel}=259$ and $\sigma_c=0.18 \sigma_u$. %For $n=512$ and $\log_2 q=28$, we have $\rho=0.682$, $n_\text{cruel}=240$ and ???.

%FC at this point results look weird: I have $\frac{\sigma}{\sigma_u}= \sqrt{h_\text{cool}\frac{\rho n - n_a}{n-n_a}}+ \frac{sigma_e}{\sigma_u} $, from Sam's Table 3, I have $n=256$, $\rho=0.779$ and $n_a=147$, if $h_\text{cool}=4$ (i.e. $h=10$), I am getting $\frac{\sigma}{\sigma_u}= 0.28 + \frac{sigma_e}{\sigma_u}$. For $n=512$, $\rho=0.693$ and $n_a=240$, with $h_\text{cool}= 5$, I am getting $\frac{\sigma}{\sigma_u}= 0.94 + \frac{\sigma_e}{\sigma_u}.$ In other words, ixsf the noise is reasonable, I can handle up to 4 cool bits in dimension 256 and 5 in dimension 512 

If all the cruel bits are correctly predicted, the variance of $x$ is $\sigma^2(x)=F_q(h_\text{cool}\sigma_c^2 + \sigma_e^2)$, where $F_q(v)$ is the variance of the composition of a centered Gaussian with a modular operation EXPLAIN WHY ASSUMED GAUSSIAN. 
If  some of the cruel bits are not correctly predicted, the variance of $x$ is $\sigma^2(x)=\sigma_u^2$.

The values of $F$, and therefore of $\sigma(x)$ can be easily tabulated (by sampling gaussian variables with the right standard deviation, and then applying the modulo $q$ operation). Table~\ref{} presents these calculations for different values of $h_cool$, for $n=256$ and $n=512$.

%Now, let $h^*$ be the number of incorrectly predicted cruel bits, and let $x = \mathbf a \cdot \mathbf s^* - b = \mathbf a \cdot (\mathbf s^* - \mathbf s)-e$. Assuming that the coordinates of $a$ remain independent after reduction, the standard deviation of $x$ is $$\sigma(x,h^*) = \sqrt{h^*} \sigma_u+\sqrt{h-h_\text{cruel}} \sigma_c+\sigma_e.$$ 
%Since $h, h_\text{cruel}, \sigma_u, \sigma_c$ and $\sigma_e$ are independent of the prediction of the cruel bits, the standard deviation is minimal when $h^*=0$, i.e. when all cruel bits are correctly predicted.

%Suppose $\sqrt{h_\text{cool}}\sigma_c + \sigma_e < \sigma_u$, 
Let us estimate $\sigma(x)$ from $m$ reduced samples, via the classical estimator 
$$\hat{\sigma} = \sqrt{\frac{1}{m-1}\sum_{i=0}^{m-1}(x_i-\overline{x})^2},$$
assuming that the Central Limit theorem holds, the upper confidence interval, with level $1-\alpha$ is
$$\iota = \hat{\sigma} \sqrt{\frac{m-1}{\chi^2_{(1-\alpha),m-1}}}$$
and we can state, with confidence $1-\alpha$, that all cruel bits are correct if $\iota < \sigma_u$.

%sNote: a weaker test could be designed by allowing up to $k$ cruel bits to be incorrect, and by enumerating all possible secrets, we would then test $\iota < \sigma(x,k) = \sqrt k \sigma_u+\sqrt{h-h_\text{cruel}} \sigma_c+\sigma_e$.

In practice, since $m$ is large, we can approximate the chi-square distribution with $m-1$ degrees of freedom by the normal distribution $\mathcal N(m-1,2m-2)$. Table~\ref{} provides estimates of $m$ at $1\%$ and $0.1\%$ confidence interval, fir different values of $q,h$ and $n$, and the reduction levels we observe in practice.

\paragraph{Testing cool bit predictions.} Once we suppose the cruel bits are correct, we need to discover the cool bits of the secret, using the algorithm~\ref{alg:greedy_cool}. We use the same test statistics as before, but in $\mathbf s^*$ the cruel bits are assumed to be correct, and the test is repeated for each cool bit of the secret.

Suppose that the $k$ first cool bits have been correctly guessed together with all the cruel bits, the secret guess $\mathbf s^*$ has the same $n_\text{cruel}+k$ first bits as the secret $\mathbf s$. The other bits in $\mathbf s^*$ are forced to zero. In the statistic $x=\mathbf a \cdot (\mathbf s^* - \mathbf s) - e$, the first  $n_\text{cruel}+k$ coordinates in the dot product are zero

%Let $s^*$ be our secret estimate, $\mathbf s$ the secret, $\mathbf  A$ the matrix of $N$ reduced vectors $\mathbf a$, and $\mathbf b=\mathbf A \cdot \mathbf s + e$. 

%(with $n_a$ the number of annoying bits). Both tests rely on comparing the standard deviations of $\mathbf A \cdot \mathbf s^* - \mathbf b = \mathbf A \cdot (\mathbf s^* - \mathbf s) + e$ if $\mathbf s^*$ is ``correct'' and if $\mathbf s^*$ is wrong. 

%Let $n_a$ be the number of annoying bits, $A_a$ the restriction

==> AFRICACRYPT_SUBMISSION/preprocess.tex <==
\section{Lattice Reduction}
\label{sec:reduction}

Here, we briefly describe the lattice reduction techniques used to produce the data in our attacks. Classical lattice reduction algorithms, such as LLL, BKZ, BKZ2.0 (\cite{LLL},\cite{CN11_BKZ},\cite{fplll})
seek to reduce the size of vectors in a lattice. 
Attacks on LWE such as the uSVP and dual attacks use 
lattice reduction algorithms to find the shortest vector, or a {\it short enough} vector, in a specifically constructed lattice.
Our attack leverages lattice reduction methods, but instead of attempting to find a single very short vector, we 
use reduced lattices as data for a distinguishing attack.
For our attack, we apply lattice reduction techniques to the embedded matrix in \cref{eq:embedding}.

Lattice reduction can be viewed as finding an integer-valued transformation matrix $\mathbf R$ which, when multiplied by $\mathbf A$ modulo $q$, reduces the Frobenius norm of $\mathbf A$. Given LWE samples in the form of a matrix $\mathbf A$ and a vector $\mathbf b =\mathbf A \cdot \mathbf s + \mathbf e$, we can use lattice reduction to reduce the entries of the matrix $\mathbf A$, yielding $\mathbf R\mathbf A$.  Then the corresponding LWE samples are ($\mathbf R\mathbf A$, $\mathbf R\mathbf b = \mathbf R\mathbf A \cdot \mathbf s + \mathbf R\mathbf e$).
Because $\mathbf R$ is applied to the noisy vector $\mathbf b$ as well, the initial noise in $\mathbf b$ is increased by the magnitude of the elements in $\mathbf R$.

For this attack, it is not always beneficial to reduce as much as possible, but rather to trade off reduction quality with the magnitude of the error $\mathbf R\mathbf e$ introduced by the reduction via the parameter $\omega$. Intuitively, the stronger the reduction, the higher the error.  The error magnitude determines the width of the blue and orange distributions in \cref{fig:as-bmodq}. \cref{sec:theory} expands on the theory which describes this trade-off.

\subsection{Our Reduction Methods}

\para{Generating sufficient LWE data.} Our attack relies on the ability to distinguish distributions from uniform, and successful distinguishing requires sufficient data. Details are discussed in \cref{sec:theory} below. An attacker might not have access to enough samples to run our attack in a real world scenario. However, sub-sampling comes to the rescue~\cite{picante}. From an initial number of $m_0$ samples, one can select a subset of $m_1$ samples, create a new $\mathbf A$ matrix, embed it in $\Lambda$, and perform lattice reduction.
This can be done many times, up to ${m_0 \choose m_1}$ times. This technique ``inflates'' the number of samples usable for this attack dramatically, at the cost of reduction of many matrices corresponding to different sub-lattices.

The SALSA Picante~\cite{picante} attack, which proposed this sub-sampling method,  eavesdrops $4n$ LWE samples, then sub-samples $n$ samples at a time and applies lattice reduction to $2n \times 2n$ q-ary matrices. 
Instead, here we sub-sample $m = \text{round}(0.875 n)$ from $4n$ LWE samples.
We then form q-ary matrices of size $(m+n) \times (m+n)$ and reduce them.

\para{Reduction algorithms.}  We leverage 3 different algorithms in our lattice reduction step: \texttt{BKZ2.0}~\cite{CN11_BKZ}, \texttt{flatter}~\cite{ryan2023fast}, and \texttt{polish}~\cite{charton2023efficient}. Each algorithm has strengths and weaknesses, and combining them maximizes the strengths of each. \texttt{BKZ2.0} provides strong reduction, but is slow for large block size and high dimensional lattices. In contrast, \texttt{flatter} is fast and can reduce lattices with $n\ge 512$ and large $q$, but only has reduction performance analogous to $\texttt{LLL}$. The \texttt{polish} algorithm runs at the end of a \texttt{flatter} or \texttt{BKZ2.0} loop~\cite{verde} and ``polishes'' by iteratively orthogonalizing matrices. It provably produces strictly decreasing vector norms when run, is implemented in C, and runs very fast.

\para{Measuring performance.} We measure lattice reduction performance via $\rho$, the ratio of the standard deviation of the entries of the reduced lattice to the expected standard deviation of the entries of a random lattice: 
\begin{align}
\rho =  \frac{\sigma(\mathbf A)}{\sigma(\mathbf A_{\text{initial}})} = \frac{\sigma(\mathbf A)}{\frac{q}{\sqrt{12}}},
\end{align}
with $\sigma(\mathbf A)$ the standard deviation of all entries of $\mathbf A$, and $\sigma(\mathbf A_{\text{initial}})$ the unreduced, original LWE sample matrix that follows a uniform distribution.
When $\rho = 1$, lattice reduction did not succeed. When $\rho \ll 1$, a significant reduction in lattice norms has been achieved. Our attack depends crucially on $\rho$, since it determines the number of cruel bits in the secret. %and the reduction on the cool bits.

\para{Interleaved reduction strategy.} Empirically, we found that combining these three algorithms gave the best reduction performance, in terms of both time and quality. \texttt{flatter} sometimes gets ``stuck'' and cannot further reduce a given lattice, particularly for smaller $q$.  In these instances, ``interleaving'' \texttt{BKZ2.0} and \texttt{flatter} provided a higher quality reduction while helping \texttt{flatter} jump out of these minima (see Table~\ref{tab:flatter_performance} for a comparison of different ways of combining \texttt{flatter} and \texttt{BKZ2.0}).  Our interleaving algorithm starts each reduction run with several rounds of \texttt{flatter} and declares a ``stall'' when \texttt{flatter} runs $3$ times  but produces an average reduction in $\rho$ of less than $0.001$. Then, the reduction runs \texttt{BKZ2.0}, and when \texttt{BKZ2.0}  stalls, it switches back to \texttt{flatter} and repeats until the reduction converges. \texttt{polish} runs after each \texttt{BKZ2.0} or \texttt{flatter} step. 


\begin{table}[h]
\vspace{-0.5cm}
\centering
\small
\caption{ 
    Comparing performance of $3$ preprocessing methods for $n=512$ and varying $\log_2 q$: \texttt{flatter} only, \texttt{flatter}-initialized BKZ (e.g. \texttt{flatter} $\rightarrow$ \texttt{BKZ}) and Interleaving. Each entry in the table reports $\rho$/hours. 
    \textbf{Bold} indicates most reduction $\rho$ with ties broken by shortest time.
    }
\resizebox{0.99\textwidth}{!}{
\begin{tabular}{ccccccccccc}
\toprule
\multicolumn{2}{c}{$\log_2 q$} & 20 & 22 & 24 & 26 & 28 & 30 & 32 & 35 & 38 \\ \midrule
\multirow{3}{*}{$\omega=4$} & Interleave & {\bf 0.77/12} & {\bf 0.75/12} & 0.72/14 & {\bf 0.69/10} & {\bf 0.67/14} & {\bf 0.64/24} & {\bf 0.57/52}& {\bf 0.50/55} &{\bf 0.44/56} \\
 & \texttt{flatter}$\rightarrow$\texttt{BKZ} & 0.81/92 & 0.79/92 & 0.76/ 92 & 0.75/114 & 0.97/72 & 0.65/109 & 0.63/55 & 0.60/63 & 0.58/60 \\
 & \texttt{flatter} only & 0.97/72 & 0.97/72 & {\bf 0.72/2} & 0.7/3 & 0.68/4 & 0.68/5 & 0.58/54 & 0.58/132 & 0.46/94 \\ \midrule
\multirow{3}{*}{$\omega=10$} & Interleave & {\bf 0.80/11} & {\bf 0.77/14} & {\bf 0.74/14} & {\bf 0.71/14} & {\bf 0.68/13} & {\bf 0.66/13} & {\bf 0.59/53} & {\bf 0.53/54} & 0.47/57 \\
 & \texttt{flatter}$\rightarrow$\texttt{BKZ} & 0.81/93 & 0.80/93 & 0.78/93 & 0.76/114 & 0.76/92 & 0.97/72 & 0.65/50 & 0.62/55 & 0.58/58 \\
 & \texttt{flatter} only & 0.97/72 & 0.97/72 & 0.97/72 & 0.72/2 & 0.69/3 & 0.68/7 & 0.62/74 & 0.58/130 & {\bf 0.46/98} \\ \bottomrule
\end{tabular}
}
\label{tab:flatter_performance}
\vspace{-0.3cm}
\end{table}


\para{Early termination.} To increase the number of reduced LWE matrices produced from a single lattice reduction run, we leverage a early termination strategy. When the standard deviation reduction ratio $\rho$ reaches some threshold $\tau$, we export the reduced matrix, then sub-sample a new $(m+n) \times (m+n)$ q-ary matrix from the initial set of $n$ LWE samples and start again. This better leverages available compute resources.


\subsection{Final Datasets} 
We apply the interleaved reduction strategy described above on the $4$ different parameter sets. %, the ``main datasets'' listed in Table \ref{tab:datasets}, additional results on two problems with larger moduli are provided in~\cref{tab:experiments_recovery} and~\cref{fig:stdev_examples}. %\emily{There are only 3 datasets in Table 4!} \nolte{@francois somewhre here should be the sentence you envision}
The number of cruel bits, $n_u$, is strongly correlated with the reduction factor $\rho$: better reduction (lower $\rho$) yields fewer cruel bits.
Because brute-forcing the $n_u$ bits is the bottleneck for our attack, we optimize the lattice reduction configuration to maximize reduction.
Reduction is trivially parallelizable, since each matrix can be processed on a different core, but is slower for larger dimensions $n$ and moduli $q$. %take longer to reduce.
% $n=1024$ takes up to XX hours for a single sample.


\begin{table}[h]
\vspace{-0.4cm}
    \centering
    \small
    \caption{
        Datasets used in concrete attacks.
        $\beta_1$ and $\beta_2$ are block sizes used in lattice reduction. 
        $\sigma_{e}$ is the ratio of standard deviation mod $q$ of the magnified error $\mathbf R\mathbf e$ to standard deviation of uniform distribution mod $q$.
        $n_u$ is the number of cruel bits. 
        We define any bits with standard deviation greater than $\frac{1}{2}\sigma(A_{\text{initial}})$ as cruel bits.
    }
    \vspace{0.1cm}
    \begin{tabular}{
        c
        c
        c
        @{\hskip 12pt}
        S[table-format=1.3]
        S[table-format=2.1]
        S[table-format=1.3]
        @{\hskip 6pt}
        S[table-format=3.0]
        @{\hskip 6pt}
        S[table-format=3.1]
    }
        \toprule
        \multicolumn{3}{c}{Inputs} & \multicolumn{5}{c}{Outputs} \\
        \cmidrule(lr){1-3} \cmidrule(lr){4-8}
        {$n$} & {$\log_2q$} & $\beta_1, \beta_2$ & {$\rho$} & {Hrs/Matrix} & {$\sigma_e$} & {$n_u$} & {$\rho^2 n$}\\
        \midrule
        \multirow{1}{*}{256} & \multirow{1}{*}{12} & \multirow{1}{*}{$35, 40$} & 0.769 & 15 & 0.952 & 143 & 151.3 \\
        % \midrule
        \multirow{1}{*}{512} & 28 & \multirow{1}{*}{$18, 22$} & 0.677 & 12 & 0.692 & 228 & 234.6 \\
        512 & 41 & $18, 22$ & 0.413 & 13.1 & 0.337 & 75 & 87.3 \\
        % & 32 & & 0.666 & 15 & 0.418 & 240 & 227.1 \\
        % \midrule
        768 & 35 & $18, 22$ & 0.710 & 15 & 0.938 & 373 & 387.1 \\
        \bottomrule
    \end{tabular}
    \vspace{-0.4cm}
    \label{tab:datasets}
\end{table}

\subsection{Quality of Reduction and Our Attack}

Experimentally we observe that the number of cruel bits, $n_u$, is roughly $\rho^2 n$.  The data sets presented in Table~\ref{tab:datasets} confirm this observation.
Intuitively, this makes sense when assuming column independence and that the standard deviation of the cool bits $\sigma_r$ is much smaller than that of the cruel bits $\sigma_u$:
\begin{align}
\sigma^2_{\text{total}} &= \frac{1}{n}(n_u \cdot \sigma_u^2 + n_r \cdot \sigma_r^2) \approx \frac{1}{n}(n_u \cdot \sigma_u^2)
\end{align}
During our experiments we usually find $\sigma_r < 0.3 \sigma_u$.


%%%%% TEXT GRAVE %%%% 
% \subsection{Lattice Reduction Algorithms}

% \para{BKZ.} The most well-known lattice reduction algorithm, LLL~\cite{LLL}, recovers an exponentially bad approximation to the shortest vector in time polynomial in the lattice dimension. A generalization of LLL, called the {\it Block Korkine-Zolotarev} method (BKZ) by Schnorr~\cite{BKZ} and Schnorr-Euchner~\cite{schnorr_euchner} improves on LLL by projecting basis vectors on sub-lattices of dimension $k < n$, where $k$ is referred to as the block size. The BKZ algorithm runs in time exponential in the block size. The block size can be increased to find shorter and shorter vectors.
%  Many improvements to BKZ have been designed and included in BKZ2.0~\cite{CN11_BKZ}, implemented in the \texttt{fplll}~\cite{fplll} library.

% \para{Flatter.} While effective at reducing lattices, BKZ is over a decade old, and the \texttt{fplll} implementation is not optimized for speed. In our experiments, we found that BKZ2.0 reduction, as implemented in \texttt{fplll}, for $n=512$, $\log_2 q=41$ can take up to weeks to converge. Recently, a new lattice reduction algorithm, \texttt{flatter}, was developed, achieving faster reduction for integer lattices ~\cite{ryan2023fast}. 
% Flatter works iteratively, first running a reduction step on a given lattice then a compression step. During the compression step, \texttt{flatter} uses careful precision management techniques to adapt the program to accommodate new int sizes as reduction progresses. This step is iterated to ensure optimal precision and minimize floating point errors. Without going too much into detail, \texttt{flatter} defines a new criterion called the drop of a lattice, and uses this criterion to track reduction success. In practice, \texttt{flatter} achieves similar performance to well-known lattice, reduction libraries, like \texttt{fplll}, but runs in a fraction of the time. It also outperforms other lattice reduction libraries that are designed to be fast, typically because those libraries tend to be very brittle or focus on a specific type of lattice.


% In our attack, we use the \texttt{flatter} Github implementation\footnote{\href{https://github.com/keeganryan/flatter}{https://github.com/keeganryan/flatter}}. 
% \texttt{flatter} does not allow for much parameter tuning, but we found that tuning the $\alpha$ parameter, described as a proxy for reduction quality, led to best results. 
% We run \texttt{flatter} with a default value of $\alpha=0.04$ and drop to $\alpha=0.025$ once reduction value dips below a certain threshold (analogous to how we increase block size and $\delta$ parameter during BKZ reduction once reduction quality reaches a certain threshold). 


% \para{The \texttt{polish} step} The final lattice reduction method considered is the polishing algorithm proposed in
% % by Charton et al
% ~\cite{charton2023efficient}. This algorithm, designed to be run at the end of an LLL or BKZ loop, ``polishes'' by iteratively orthogonalizing matrices. \texttt{polish} 
% % as we will refer to it going forward, 
% is proven to produce strictly decreasing vector norms whenever it is run. It is implemented in C and runs in negligible time.


%We compare the performance of the three previously described reduction methods (e.g. \texttt{BKZ}, \texttt{flatter}, \texttt{polish}), as well as combinations of these methods. 

% We experimented with \texttt{flatter} as a stand-alone algorithm as well as combining \texttt{flatter} with \texttt{BKZ} in two different ways: using \texttt{flatter} to initialize \texttt{BKZ}; and interleaving \texttt{flatter} with \texttt{BKZ}.
% \texttt{flatter}-initialized \texttt{BKZ} runs one round of \texttt{flatter} before reverting to \texttt{BKZ} for rest of preprocessing. 
% Table~\ref{tab:flatter_performance} shows the timings and reduction quality produced by these three \texttt{flatter}-based reduction methods, for $n=512$ with various $\log_2 q$ and two different reduction penalty parameters $\omega$.


% All three reduction methods were allowed to run for the same amount of time. 
% We measured $\rho$ and the time required to reduce (denoted as $\rho$/hours in the table). Entries for which $\rho$ is high but ``hours'' is low typically indicate that reduction got ``stuck'' and could not progress beyond this point, despite running for several days. Overall, we found that \texttt{flatter} significantly improved processing time for $n=512$, while achieving similar reduction quality as BKZ alone. Reduction times for dimension $n=512$ lattices are given in terms of hours in Table~\ref{tab:flatter_performance}. 

% % KL: commented out to maintain anonimity 
% % We do not report comparison points of \texttt{BKZ} because it takes more than $3$ days to run for the $\log_2 q$ values tested, resulting in the job being automatically shut down by our compute cluster.

%When processing 1 matrix, this method only produces $2n$ samples at the end, after hours or days of lattice reduction. To produce a dataset, it uses a lot of CPUs. To glean more reduced samples from each lattice reduction run, we revise the preprocessing algorithm to start writing data once $\sigma_{red}$ reaches some threshold $\tau + \epsilon$ for a very small $\epsilon > 0$. We then let each CPU keep reducing a given matrix and writing off new data as long as $\tau - \epsilon < \sigma_{red} < \tau + \epsilon$. This means that $k(m+n)$ samples are harvested from each CPU/matrix run, where $k$ (typically $k>>1$) depends on how many reduction steps the CPU must go through to get $\sigma_{red}$ from $\tau + \epsilon$ to $\tau - \epsilon$. 
%\sam{We actually don't do this in this paper because of the data.prefix issue. Maybe we save this for a later paper. (NN) yes, esp because we still don't know whether that kind of data helps us!}
 

% \para{Results.} Table~\ref{tab:reduce_compute} shows preprocessing performance using these improved sampling and compute techniques for $n=256$, $\log_2 q = 12$. The $\rho$ achieved
%which is the proportionate reduction in matrix standard deviation as a result of preprocessing (smaller $\sigma_{red}$ indicates stronger reduction), 
% is roughly the same with both sampling methods. 
% The {\em \# matrices to write} is slightly larger for the method starting with $n$ initial samples, due to smaller matrix size (fewer rows in one matrix) and duplicates produced by exporting at multiple stages when processing the same matrix. The wall time is slightly larger because for each matrix, $\rho$ needs to reach $\tau - \epsilon$ instead of $\tau$. However, the {\em \# of matrices to process} is {\em much} smaller when initial number of samples is $n$, due to this $\tau/\epsilon$ thresholding method, highlighting the significant reduction in compute requirements. 

% \begin{table}[h]
%     \small
%     \centering
%     \caption{{\bf Effect of starting with $n$ vs. $4n$ samples and writing once $\rho$ reaches threshold $\tau + \epsilon > \tau$ on preprocessing time}: {\em \# mat to write}: the number of matrices needed to produce 4M sample dataset\sout{; {\em wall time}: time to run if fully parallelized}.}
%     \begin{tabular}{
%         c
%         S[table-format=1.3]
%         S[table-format=5.0]
    
%     }
%         \toprule
%         \# orig samples & $\rho$ & \# mat to write & \# mat to process & hrs/matrix & total CPU.hrs  \\ 
%         \midrule
        
%         $4n$ (1024) & 0.767 & 10800 & 10800 & 1.6 hrs & 17280 \\
%         $n$ (256) & 0.769 & 12000 & 500 & 2.4 hrs & 1200  \\ 
%         \bottomrule
%     \end{tabular}
%     \label{tab:reduce_compute}
% \end{table}

==> AFRICACRYPT_SUBMISSION/recovery.tex <==

\begin{table}[t]
\vspace{-0.3cm}
    \centering
    \small
    \caption{
        Concrete attacks on different secrets: 
        $n = $ dimension, $\log_2 q$ is the modulus size, 
        $h = $ Hamming weight of the secret. 
        $h_u$ indicates the number of cruel bits which are $1$. 
        \% and cumulative \% measure how many secrets with hamming weight $h$ have $h_u$ bits and $h_u$ bits or fewer, respectively.
        We run all attacks on one GPU to be comparable, but also demonstrate scaling in the toughest setting to 20 GPUs.
    }
    \vspace{0.1cm}
    \begin{tabular}{ccccccc}
        \toprule
        $n$ & $\log_2 q$ \quad & $h$ & $h_u$ & \quad \% (cum. \%) \quad & Samples Used & \quad Time (1 V100 GPU) \\
        \midrule
        \multirow{4}{*}{256} & \multirow{4}{*}{12} & 12 & 4 & 6.7 (9.5) & \multirow{4}{*}{200K} & 28\,s \\
        & & 12 & 5 & 14.1 (23.6) & & 84\,s, 241\,s \\
        & & 12 & 6 & 21.2 (44.8) & & 3865\,s, 4098\,s \\
        & & 12 & 7 & 23.0 (67.8) & & 23229\,s, 26229\,s \\
        \midrule
        % \multirow{5}{*}{256} & \multirow{5}{*}{20} & 40 & 4 & 9.9 (16.9) & \multirow{5}{*}{1M} & 41\,s \\
        % & & 40 & 6 & 18.2 (50.3) & & 57\,s \\
        % & & 40 & 7 & 17.6 (67.9) & & 70\,s, 94\,s \\
        % & & 40 & 8 & 13.9 (81.8) & & 144\,s, 273\,s \\
        % & & 40 & 10 & 5.1 (96.1) & & 2904\,s \\
        % \midrule
        \multirow{3}{*}{512} & \multirow{3}{*}{28} & 12 & 3 & 9.5 (13.9) & \multirow{3}{*}{200K} & 29\,s \\
        & & 12 & 4 & 17.5 (31.4) & & 70\,s \\
        & & 12 & 5 & 22.7 (54.0) & & 2417\,s, 3510\,s \\ 
        \midrule
        \multirow{2}{*}{512} & \multirow{2}{*}{41} & 60 & 7 & 16.6 (53.6) & \multirow{2}{*}{1M} & 376\,s, 341\,s \\
        & & 60 & 8 & 15.5 (69.1) & & 1555\,s \\
        \midrule
        \multirow{4}{*}{768} & \multirow{4}{*}{35} & 10 & 3 & 13.1 (19.5) & \multirow{4}{*}{200K} & 165\,s, 168\,s \\
        & & 10 & 4 & 21.7 (41.2) & & 269\,s, 745\,s \\
        \cmidrule(lr){3-4}
        & & 12 & 4 & 13.5 (22.1) & & 607\,s, 688\,s \\
        & & 12 & 5 & 20.5 (42.6) & & 1291\,s (scaled to 20 GPUs) \\
        \bottomrule
    \end{tabular}
    \vspace{-0.4cm}
    \label{tab:experiments_recovery}
\end{table}


\section{Recovery Results}
\label{sec:results}

In this section we provide concrete performance results for our attacks.
We run the attack as described in Section \ref{sec:practical} for different LWE parameter settings and report results in Table~\ref{tab:experiments_recovery}. After reduction, the running time depends almost entirely on the amount of enumeration that has to be done on the cruel bits.
Enumeration is done in ascending hamming weight on those bits.
We extend the secret to the cool bits via the greedy algorithm, every 40M secret candidates, or whenever completing the enumeration on one hamming weight.

All times reported in Table \ref{tab:experiments_recovery} include the compilation time during the first run over a secret, which is of the order of 10 seconds, and loading data, also of the order of 10 seconds. For some secrets, we report multiple timings to illustrate that the process is somewhat noisy, mostly depending on where in the enumeration the secret happens to be.
For the settings with higher hamming weights ($h=60$), we use 200k samples for the brute force attack and 1M for the greedy attack. For the lower hamming weights, we use 10k-30k samples for the brute force attack and 200k for the greedy part.


\para{Existing attacks.} For completeness, we compare the performance of our attack to prior work. The hybrid dual meet-in-the-middle (MiTM) attack is most similar to ours~\cite{Cheon_hybrid_dual}, but options for comparison against this are limited, since no concrete performance results are provided in~\cite{Cheon_hybrid_dual}. Some concrete performance results are given for related attacks, but ~\cite{albrecht2017revisiting} only consider $n \le 110$ and $\log q = 11$,~\cite{postlethwaite2021success} considers $n \le 100$ and $\log q = 8$. Thus, we choose two routes for comparison. First, we compare against estimated cost of the hybrid dual MiTM estimate from the LWE estimator tool\cite{LWEestimator}, and then we compare against a recent concrete attack implementation for sparse secret LWE proposed by~\cite{rumpsession}. The latter has code available\footnote{https://github.com/lducas/leaky-LWE-Estimator/tree/human-LWE/human-LWE} and claims to be fast. It provides a MITM attack in Python for the $n=256$, $\log q=12$ setting and a modified uSVP/BDD attack for larger parameters.

Table~\ref{tab:other_attacks} reports these results. For the estimator~\cite{LWEestimator}, we report the estimated number of operations, the memory required, and the number of attack repeats required to achieve a $1-10^{-5}$ probability of success (to match our $\alpha$, $\beta$ levels in \S\ref{sec:theory}). We convert the predicted memory into bytes by multiplying estimator output (number of integers to be stored) by number of bits required to store this integer ($32$ is suggested).  We note that the ROP metric reported by the estimator is a crude estimate for runtime, since it refers to the number of comparisons or operations necessary for the attack to run, which does not easily translate to a fixed time metric. For~\cite{rumpsession}, we report time to successful attack, if it succeeds. A `-' in the column indicates the attack ran for $>24$ hours without finishing.
%As Table~\ref{tab:other_attacks} shows, for settings $n > 256$, our attack runs faster than~\cite{rumpsession}, requires no repeats to increase probability of success, and requires significantly less memory than the Hybrid MiTM attack, at the expense of more compute. 
\begin{table}[h]
\vspace{-0.6cm}
\centering
\caption{Estimates of Dual Hybrid MiTM performance~\cite{LWEestimator} and concrete attack performance by~\cite{rumpsession} at parameter settings explored in this work. ROP = estimated number of required operations for attack, Memory = estimated memory required for MiTM hash table, Repeats = $\#$ of times attack must run to succeed with probability $0.99999$.}
\vspace{0.1cm}
\label{tab:other_attacks}
    \setlength{\tabcolsep}{8pt}
\begin{tabular}{ccccc}
\toprule
\multirow{2}{*}{ 
\textbf{\begin{tabular}[c]{@{}c@{}}LWE setting\\ ($n,q,h$)\end{tabular}}} & \multicolumn{3}{c}{\textbf{Hybrid MiTM Dual~\cite{LWEestimator}}} & \textbf{Ducas et al}~\cite{rumpsession} \\ 
 & ROP & Memory & Repeats & Time (sec)  \\ \midrule
$(256,12,12)$ & $2^{50.2}$ & $3.3$TB & $2^{13.6}$ & 200 \\
$(512, 28,12)$ & $2^{48.3}$ & $2.05$TB & $2^{10.4}$ &  - \\
$(512, 41, 60)$ & $2^{50.4}$ & $10.8$TB & $2^{7.1}$ &  - \\
$(768, 35, 12)$ & $2^{48.8}$ & $725$GB & $2^{10.6}$ & -  \\ \bottomrule
\end{tabular}
\vspace{-0.2cm}
\end{table}



% We calculate the probability of a secret with Hamming weight $h$ having $h_u$ ones in the $n_u$ cruel bits:
% \begin{equation}
%     \frac{{h_u \choose n_u}{h_r \choose n_r}}{{n \choose h}}
% \end{equation}


==> AFRICACRYPT_SUBMISSION/rlwe.tex <==
\section{2-power cyclotomic Ring-LWE}
\label{sec:RLWE}

Our attack can also be applied in the 2-power cyclotomic Ring-LWE setting.
Ring-LWE (RLWE) is a special case of LWE where the LWE samples can be represented more compactly as polynomials in a polynomial ring.
Not all instances of Ring-LWE are hard, as was shown in~\cite{ELOS}. But $2$-power cyclotomic rings are not vulnerable to the attack in~\cite{ELOS}, so those are the rings standardized for use in Homomorphic Encryption~\cite{HES}. 

Consider the $2$-power cyclotomic ring defined by the polynomial $x^n+1$, where $n=2^k$: $R_q = \mathbb{Z}_q[X]/(X^n+1)$.
Then the RLWE samples corresponding to a polynomial RLWE sample, $(a(x), b(x) = a(x) \cdot s(x) + e(x))$ can be described via a skew-circulant matrix, $\mathbf A_{circ}$.  
If $a(x) = a_0 + a_1x + ... + a_{n-1}x^{n-1}$, then:
\[
\mathbf A_{\text{circ}} =  \begin{bmatrix}
a_0 & -a_{n-1} & -a_{n-2} &\dots & -a_1 \\
a_1 & a_0 & -a_{n-1} & \ddots & -a_2 \\
\vdots & a_1 & a_0 & \ddots & -a_{n-1} \\
a_{n-1} & \ddots & \ddots & \ddots & a_0
\end{bmatrix}
\]
and $\mathbf b_{\text{circ}} = \mathbf A_{\text{circ}} \mathbf s + \mathbf e$ where $\mathbf s$ and $\mathbf e$ are the vector representations of $s(x)$ and $e(x)$ respectively.

When the matrix has this structure, we can rotate the ``cruel bits'' around (without redoing any lattice reduction) and increase our chances of recovering the secret, if there are only a small number of cruel bits in one of the rotated cruel regions.  This makes the RWLE problem clearly easier than generic LWE in those cases, with respect to our attack.

Let $\mathbf A \in \mathbb{Z}_q^{m\times n}$ be the reduced samples; $\mathbf A = \mathbf{RA}_{\text{circ}}  \text{ for some } \mathbf R\in \mathbb{Z}^{m\times n}$. We can shift-negate the reduced samples $k$ times to get new samples  $(\mathbf A^{\leftarrow k}, \mathbf b^{\leftarrow k})$ (see \ref{sec:appx}). The attack for RLWE consists of performing brute force on $n$ sliding windows $[k,k+n_u\mod n)$ simultaneously (or any other number of windows by using a higher sliding step). The exhaustive search will cover less search space as we only need to check up to $h^{(1)}_u = \min_{0 \leq i<n} h_{n_u, i}(\mathbf s)$ hamming weight where 
\begin{align}
    h_{n_u, i}(\mathbf s) = \sum_{j=i}^{i+n_u-1[n]} s_j
    \label{eq:hui}
\end{align}

In this context, $h_{n_u, i}(\mathbf s)$ represents the Hamming weight of a specific segment of the secret vector $\mathbf s$, starting at position $i$ and of length $n_u$. It's important to note that when $i=0$, this notation aligns with our previous use of $h_u$ to denote the Hamming weight of the first $n_u$ elements of $\mathbf s$. Similarly, when $n_r=n-n_u$, $h_{n_r, n_u}(\mathbf s)$ aligns with our previous use of $h_r$ to denote the Hamming weight of the last $n_r=n-n_u$ elements of $\mathbf s$.

To evaluate the speed up of this attack compared to the LWE case, we estimate the cost of the brute force component while assuming equal cost of the lattice reduction for LWE and RLWE. Let $c\cdot M(h_r(s), \alpha, \beta)$ represent the cost of checking a secret candidate using $M(h_r(s), \alpha, \beta)$ samples, where $c$ is a constant factor that accounts for the computational resources required for each verification. 
The average time complexity of the exhaustive search for LWE, assuming we sweep through the secret candidates in ascending Hamming weight order, is:
$$T_{\text{guess}}^{\text{LWE}} = \mathbb{E}_s\Biggl [c\cdot M(h_r(s), \alpha, \beta)\sum_{k=0}^{h_u(s), } \binom{n_u}{k}\Biggr]$$

\noindent By using the same amount of samples $M=M(h_r(s), \alpha, \beta)$ in the attack for all secret candidates, we have 
$$T_{\text{guess}}^{\text{LWE}} = c\cdot M\cdot \sum_{k=0}^{h} \binom{n_u}{k}\mathbb{P}(h_u(s) \geq k)$$

\noindent In the RLWE case, we have $\mathbb{P}(h^{(1)}_u \leq \frac{hn_u}{n}) = 1$ so that \[
T_{\text{guess}}^{\text{RLWE}}  = n\cdot c\cdot M\cdot \sum_{k=0}^{\lfloor \frac{hn_u}{n}\rfloor} \binom{n_u}{k}\mathbb{P}(h^{(1)}_u \geq k)
\]
\begin{figure}[t]
    \centering
    \includegraphics[width=0.5\linewidth]{figs/ratio_T.pdf}
    \vspace{-0.1cm}
    \caption{Exhaustive search cost ratio for LWE versus RLWE assuming a fixed $10\%n$ binary secret sparsity. The values of $n_u$ are obtained experimentally.}
    \label{fig:rlwe_tguess_ratio}
    \vspace{-0.4cm}
\end{figure}

In \cref{fig:rlwe_tguess_ratio}, we estimate the ratio of the costs above. Note that the distribution of $h_u(s)$ conditionally to a fixed total hamming weight $h$ follows a hyper-geometric distribution when the secret bits are from Bernoulli, while the $h^{(1)}_u$ distribution is computed empirically.

We conduct several experiments comparing LWE with RLWE, using identical secrets for comparison. The results of these experiments, for parameters $n=256$ and $n=512$, are presented in \cref{tab:n256} and \cref{tab:n512}. Each table row corresponds to a distinct secret $s$, and the columns detail the actual and estimated time costs for the LWE and RLWE attacks, along with the count of cruel bits in the secret. In the tables, Actual Time is the empirically measured duration of the attack, while the Estimated Time is estimated using an approximation $T_{\text{guess}}^{\text{LWE}} = b + a\sum_{k=0}^{h_u(s)} \binom{n_u}{k}$. This estimation provides an idea of the time required to attack a secret with high $h_u$, a process that would demand substantial computational resources in a practical setting. 


Note that for RLWE, the Time is multiplied by $n$ to account for the increased complexity of running multiple brute force attacks simultaneously, which can be optimized. The final row provides the average values across all secrets. As can be seen, the RLWE attack is significantly faster on average, with the ratio of average times being $\sim 10^3$ for $n=256$ and $5\times 10^3$ for $n=512$, but converge to the theoretical values in \cref{fig:rlwe_tguess_ratio} when estimated on more secret samples. The RLWE advantage can also be seen in the values of $h^{(1)}_u(s)$ which are much smaller than those of $h_u(s)$. 

\begin{table}[t]
\vspace{-0.4cm}
    \caption{Attack times for parameters: $n = 256, h = 12, \log Q = 12, n_u = 145$ run on 20 randomly sampled secrets. Actual time is the empirical time of the attack. Estimated time is computed via the formula: $T_{\text{guess}}^{\text{LWE}} = b + a\sum_{k=0}^{h_u(s)} \binom{n_u}{k}$ and $T_{\text{guess}}^{\text{RLWE}} = n(b + a\sum_{k=0}^{h^{(1)}_u} \binom{n_u}{k})$ for RLWE. $h_u(s)$, as defined in \cref{eq:hui}, is the number of the cruel bits of the secret, and $h^{(1)}_u$ is the minimum hamming weight over all windows of length $n_u$. We use $56k$ samples for Cruel bit recovery and $200k$ for \cref{alg:greedy_cool}. }%Ratio of time averages over 20 secrets $\frac{T^{LWE}}{T^{RLWE}}=1041$}
    \vspace{0.1cm}
    \centering
    \small
    \setlength{\tabcolsep}{5pt}
    \begin{tabular}{ccccccc}
\toprule
 & \multicolumn{3}{c}{LWE}  & \multicolumn{3}{c}{RLWE}  \\
\cmidrule{2-7}
 Secret & Estimated & Actual & &  Estimated &Actual &  \\
 & time (sec) & time (sec) & $h_u(s)$ &    time & time&$h^{(1)}_u(s)$\\
\midrule
1 & $2.33\times 10^1$ & $2.21\times 10^1$ & 3 & $5.86\times 10^3$ & $4.83\times 10^3$ & 2 \\
2 & $4.60\times 10^2$ & $3.59\times 10^2$ & 5 & $1.18\times 10^5$ & $1.21\times 10^5$ & 5 \\
3 & $4.60\times 10^2$ & $5.24\times 10^2$ & 5 & $1.18\times 10^5$ & $1.73\times 10^5$ & 5 \\
4 & $4.60\times 10^2$ & $4.12\times 10^2$ & 5 & $9.77\times 10^3$ & $1.02\times 10^4$ & 4 \\
5 & $4.60\times 10^2$ & $2.61\times 10^2$ & 5 & $5.97\times 10^3$ & $4.58\times 10^3$ & 3 \\
6 & $4.60\times 10^2$ & $3.61\times 10^2$ & 5 & $9.77\times 10^3$ & $1.19\times 10^4$ & 4 \\
7 & $1.04\times 10^4$ & -- & 6 & $5.97\times 10^3$ & $6.00\times 10^3$ & 3 \\
8 & $2.09\times 10^5$ & -- & 7 & $1.18\times 10^5$ & $1.76\times 10^5$ & 5 \\
9 & $2.09\times 10^5$ & -- & 7 & $1.18\times 10^5$ & $1.48\times 10^5$ & 5 \\
10 & $2.09\times 10^5$ & -- & 7 & $9.77\times 10^3$ & $1.20\times 10^4$ & 4 \\
11 & $2.09\times 10^5$ & -- & 7 & $9.77\times 10^3$ & $1.15\times 10^4$ & 4 \\
12 & $2.09\times 10^5$ & -- & 7 & $5.97\times 10^3$ & $5.71\times 10^3$ & 3 \\
13 & $2.09\times 10^5$ & -- & 7 & $1.18\times 10^5$ & $5.38\times 10^4$ & 5 \\
14 & $3.66\times 10^6$ & -- & 8 & $9.77\times 10^3$ & $1.06\times 10^4$ & 4 \\
15 & $3.66\times 10^6$ & -- & 8 & $9.77\times 10^3$ & $1.26\times 10^4$ & 4 \\
16 & $3.66\times 10^6$ & -- & 8 & $9.77\times 10^3$ & $1.19\times 10^4$ & 4 \\
17 & $5.65\times 10^7$ & -- & 9 & $5.97\times 10^3$ & $4.12\times 10^3$ & 3 \\
18 & $5.65\times 10^7$ & -- & 9 & $1.18\times 10^5$ & $1.33\times 10^5$ & 5 \\
19 & $5.65\times 10^7$ & -- & 9 & $5.97\times 10^3$ & $6.02\times 10^3$ & 3 \\
20 & $7.81\times 10^8$ & -- & 10 & $5.86\times 10^3$ & $4.74\times 10^3$ & 2 \\
\midrule
Avg & $4.81\times 10^7$ & $9.63\times 10^1$ & $6.85\times 10^0$ & $4.08\times 10^4$ & $4.61\times 10^4$ & $3.85\times 10^0$ \\
\bottomrule
\end{tabular}
\label{tab:n256}
\vspace{-0.3cm}
\end{table}

\begin{table}[t]
\vspace{-0.3cm}
    \caption{Attack times (in seconds) and estimated costs for $n=512, n_u=75, h=60, \log Q = 41$ for random $20$ secrets sorted by number of secret cruel bits in LWE. We use $40K$ samples for cruel bit recovery and $1.5M$ for \cref{alg:greedy_cool} }
    \vspace{0.1cm}
    \centering
    \small
    \setlength{\tabcolsep}{5pt}
    \begin{tabular}{ccccccc}
    \toprule
     & \multicolumn{3}{c}{LWE}  & \multicolumn{3}{c}{RLWE}  \\
    \cmidrule{2-7}
     Secret & Estimated & Actual & &  Estimated &Actual &  \\
     & time (sec) & time (sec) & $h_u(s)$ &    time & time&$h^{(1)}_u(s)$\\
    \midrule
    1 & $6.88\times 10^2$ & $5.95\times 10^2$ & 6 & $1.82\times 10^5$ & $7.74\times 10^4$ & 4 \\
    2 & $6.88\times 10^2$ & $2.82\times 10^3$ & 6 & $1.95\times 10^5$ & $6.31\times 10^4$ & 5 \\
    3 & $3.98\times 10^3$ & $3.93\times 10^3$ & 7 & $1.82\times 10^5$ & $7.68\times 10^4$ & 4 \\
    4 & $3.45\times 10^4$ & -- & 8 & $3.52\times 10^5$ & $1.08\times 10^5$ & 6 \\
    5 & $2.82\times 10^5$ & -- & 9 & $1.82\times 10^5$ & $4.62\times 10^4$ & 4 \\
    6 & $2.82\times 10^5$ & -- & 9 & $1.82\times 10^5$ & $5.01\times 10^4$ & 4 \\
    7 & $2.82\times 10^5$ & -- & 9 & $1.95\times 10^5$ & $8.72\times 10^4$ & 5 \\
    8 & $2.82\times 10^5$ & -- & 9 & $1.95\times 10^5$ & $1.15\times 10^6$ & 5 \\
    9 & $2.06\times 10^6$ & -- & 10 & $3.52\times 10^5$ & -- & 6 \\
    10 & $2.06\times 10^6$ & -- & 10 & $1.82\times 10^5$ & $4.64\times 10^4$ & 4 \\
    11 & $2.06\times 10^6$ & -- & 10 & $1.81\times 10^5$ & -- & 3 \\
    12 & $2.06\times 10^6$ & -- & 10 & $1.81\times 10^5$ & -- & 2 \\
    13 & $1.36\times 10^7$ & -- & 11 & $1.82\times 10^5$ & $6.21\times 10^4$ & 4 \\
    14 & $1.36\times 10^7$ & -- & 11 & $1.95\times 10^5$ & $9.58\times 10^4$ & 5 \\
    15 & $1.36\times 10^7$ & -- & 11 & $1.82\times 10^5$ & -- & 4 \\
    16 & $1.36\times 10^7$ & -- & 11 & $1.82\times 10^5$ & $3.56\times 10^4$ & 4 \\
    17 & $8.06\times 10^7$ & -- & 12 & $1.81\times 10^5$ & $4.43\times 10^4$ & 3 \\
    18 & $4.36\times 10^8$ & -- & 13 & $1.82\times 10^5$ & -- & 4 \\
    19 & $9.88\times 10^9$ & -- & 15 & $1.81\times 10^5$ & $4.46\times 10^4$ & 3 \\
    20 & $9.88\times 10^9$ & -- & 15 & $1.81\times 10^5$ & $4.67\times 10^4$ & 2 \\
    \midrule
    Avg & $1.02\times 10^9$ &  & $10.1$ & $2.01\times 10^5$ &  & $4.05$ \\
    \bottomrule
    \end{tabular}
    \label{tab:n512}
    \vspace{-0.3cm}
\end{table}






==> AFRICACRYPT_SUBMISSION/tables/Table5removed.tex <==
 \begin{table}[h]
    \small
    \centering
    \caption{\small \textbf{Cruel bit recovery.} Ratio of standard deviations that the test can recover (lower confidence bound), for different pre-processed sample sizes and confidence levels. \nolte{this does not fit with the formula}}
    \label{tab:cruelconfidence}
    \begin{tabular}{ccccccccc}
        \toprule
        & \multicolumn{8}{c}{Sample size (m)}\\
        Confidence level & 1,000 & 5,000 & 10,000 & 50,000 & 100,000 & 500,000 & 1,000,000 & 5,000,000 \\
        \midrule
        $\alpha=10^{-2}$ & $0.952$ & 0.978  & 0.984 & 0.993 & 0.995 & 0.998 & 0.998 & 0.999 \\ 
        $\alpha=10^{-3}$ & 0.937 & 0.970  & 0.979 & 0.990 & 0.993 & 0.997 & 0.998 & 0.999 \\
        $\alpha=10^{-6}$ & 0.908 & 0.956  & 0.968 & 0.985 & 0.990 & 0.995 & 0.997 & 0.999\\
        $\alpha=10^{-9}$& 0.888 & 0.945  &  0.960 & 0.982 & 0.987 & 0.994 & 0.996 & 0.998\\
        $\alpha=10^{-12}$ & 0.872 & 0.936  & 0.954 & 0.978 & 0.985 & 0.993 & 0.995 & 0.998 \\
        $\alpha=10^{-15}$ & 0.859 & 0.929  & 0.948 & 0.976 & 0.983 & 0.992 & 0.994 & 0.997 \\

       \bottomrule
    \end{tabular}
%    \vspace{-0.5cm}
\end{table}



==> AFRICACRYPT_SUBMISSION/tables/notation.tex <==

\begin{table}[h]
\vspace{-0.7cm}
    \centering
    \small
    \caption{Notation used in this paper.}
    \begin{tabular}{c@{\hskip 6pt}l}
        \toprule
        Symbol & Description \\
        \midrule
        $q$ & The modulus of the LWE problem considered \\
        $n$ & Problem dimension (the dimension of vectors $\mathbf a$ and $\mathbf s$) \\
        $n_u$ & The number of unreduced (aka cruel) entries in $\mathbf a$. \\
        $n_r$ &  Number of reduced (aka cool) entries in $\mathbf a$.  $n = n_u + n_r$ \\
        $\mathbf s$ & The unknown secret, used to construct $b=\mathbf a \cdot \mathbf s + e$ \\
        $\mathbf s^*$ & A candidate secret, not necessarily correct \\
        $h$ & The Hamming weight of the secret (number of 1 bits) \\         
        $h_u$ & The Hamming weight of the $n_u$ unreduced bits of the secret \\
        $h_r$ & The Hamming weight of the $n_r$ reduced bits of the secret ($h=h_u+h_r$)\\
        $\sigma_u$ & The standard deviation of unreduced entries in $\mathbf a$ (equal to $\frac{q}{\sqrt{12}}$) \\
        $\sigma_r$ & The standard deviation of reduced entries in $\mathbf a$ \\
        $\sigma_e$ & The standard deviation of error (amplified by reduction) \\
        $\sigma(x)$ & The standard deviation of the random variable $x$ \\
        $\rho$ & The reduction factor of pre-processing, i.e. the ratio $\frac {\sigma(\mathbf R \mathbf A)}{\sigma(\mathbf A)}$ \\ %of the standard deviation of $\mathbf A$ (before reduction) and $\mathbf RA$ (i.e. after reduction) \\ 
        $m$ & The number of LWE samples (reduced or unreduced) \\
        $\omega$ & The penalty used during reduction \\
        $a:b$ & integer range $[a, b)$, used for indices \\
        $\mathbf{X}_{*,i}$ & $i$th column of $\mathbf X$ \\
        %$\mathbf{s}_{\text{true}}$ &  The true secret used to construct $b$. \\
        %$\mathbf{s}_{\text{cand}}$ &  A candidate secret; not necessarily the true secret. \\
        \bottomrule
    \end{tabular}
    \label{tab:notation}
    \vspace{-0.3cm}
\end{table}


==> AFRICACRYPT_SUBMISSION/tables/params.tex <==
\begin{table}[h!]
\vspace{-4mm}
\small
  \centering
    \small\caption{\textbf{\lwe{}, preprocessing, and training parameters}. For the adaptive increase of preprocessing parameters, we start with blocksize $\beta_1$ and LLL-delta $\delta_{LLL1}$, and upgrade to $\beta_2$ and $\delta_{LLL2}$ at a later stage. Parameters base $B$ and bucket size $r$ are used to tokenize the numbers for transformer training. }
    \label{tab:params}
      \vspace{2mm}
\begin{tabular}{lllllllll}
\toprule
$n$                    & $\log_2 q$ & $q$             & $\beta_1$ & $\delta_{LLL1}$ & $\beta_2$ & $\delta_{LLL2}$ & base $B$         &  bucket size $r$         \\ \midrule
 \multirow{5}{*}{256} & 12   & 3329          & 35   & 0.99  & 40   & 1     & 417          & 1         \\
                     & 14   & 11197         & 35   & 0.99  & 40   & 1     & 1400         & 1         \\
                     & 16   & 42899         & 35   & 0.99  & 40   & 1     & 5363         & 4         \\
                     & 18   & 222553        & 35   & 0.99  & 40   & 0.99  & 27820        & 16        \\
                     & 20   & 842779        & 35   & 0.99  & 40   & 0.99  & 105348       & 64        \\ \midrule
\multirow{2}{*}{350} & 21   & 1489513       & 30   & 0.96  & 40   & 0.99  & 186190       & 128       \\
                     & 27   & 94056013      & 30   & 0.96  & 40   & 0.99  & 5878501      & 4096      \\ \midrule
512                  & 41   & 2199023255531 & 18   & 0.93  & 22   & 0.96  & 137438953471 & 134217728 \\ \bottomrule
\end{tabular}
\end{table}

==> AFRICACRYPT_SUBMISSION/theory.tex <==
\section{Theoretical Analysis of Attack Time}

We analyze the run time of this attack according to its three stages.

\begin{enumerate}
\item Stage 1: lattice reduction of matrix $A$ using flatter or BKZ 2.0 to achieve std deviation $\sigma$
We use the same cost model for this step as is used in \cite{Cheon_hybrid_dual} to make the comparison easier.  See cost model described in Lattice section above.

\item  Stage 2: For a data set with std deviation $\sigma$ we expect to have approximately $k = \sigma^2 n$ cruel bits.  See Heuristic described above/below and Table~\ref{?} for experimental evidence.
We run through all possible secrets starting with the lowest possible Hamming weight, and increasing the Hamming weight one by one.  This step considers at most (k choose h) secrets.

\item Stage 3: A statistical test is applied to all possible secrets of length $k$.  The cost of the statistical test is proportional to (?) the number of samples needed for the test.




\end{enumerate}


{\bf Heuristic}: For a data set reduced via lattice reduction techniques such as flatter or BKZ2.0, with std deviation $\sigma$, we expect to have approximately $\sigma^2 n$ cruel bits.


==> tables/params.tex <==
\begin{table}[h!]
\vspace{-4mm}
\small
  \centering
    \small\caption{\textbf{\lwe{}, preprocessing, and training parameters}. For the adaptive increase of preprocessing parameters, we start with blocksize $\beta_1$ and LLL-delta $\delta_{LLL1}$, and upgrade to $\beta_2$ and $\delta_{LLL2}$ at a later stage. Parameters base $B$ and bucket size $r$ are used to tokenize the numbers for transformer training. }
    \label{tab:params}
      \vspace{2mm}
\begin{tabular}{lllllllll}
\toprule
$n$                    & $\log_2 q$ & $q$             & $\beta_1$ & $\delta_{LLL1}$ & $\beta_2$ & $\delta_{LLL2}$ & base $B$         &  bucket size $r$         \\ \midrule
 \multirow{5}{*}{256} & 12   & 3329          & 35   & 0.99  & 40   & 1     & 417          & 1         \\
                     & 14   & 11197         & 35   & 0.99  & 40   & 1     & 1400         & 1         \\
                     & 16   & 42899         & 35   & 0.99  & 40   & 1     & 5363         & 4         \\
                     & 18   & 222553        & 35   & 0.99  & 40   & 0.99  & 27820        & 16        \\
                     & 20   & 842779        & 35   & 0.99  & 40   & 0.99  & 105348       & 64        \\ \midrule
\multirow{2}{*}{350} & 21   & 1489513       & 30   & 0.96  & 40   & 0.99  & 186190       & 128       \\
                     & 27   & 94056013      & 30   & 0.96  & 40   & 0.99  & 5878501      & 4096      \\ \midrule
512                  & 41   & 2199023255531 & 18   & 0.93  & 22   & 0.96  & 137438953471 & 134217728 \\ \bottomrule
\end{tabular}
\end{table}
